Space-time finite element analysis of the advection-diffusion equation using Galerkin/least-square stabilization

We present a full space-time numerical solution of the advection-diffusion equation using a continuous Galerkin finite element method on conforming meshes. The Galerkin/least-square method is employed to ensure stability of the discrete variational problem. In the full space-time formulation, time is considered another dimension, and the time derivative is interpreted as an additional advection term of the field variable. We derive a priori error estimates and illustrate spatio-temporal convergence with several numerical examples. We also derive a posteriori error estimates, which coupled with adaptive space-time mesh refinement provide efficient and accurate solutions. The accuracy of the space-time solutions is illustrated against analytical solutions as well as against numerical solutions using a conventional time-marching algorithm.

==> extras/6_15z_comparison_sequential_1x.tex <==
\begin{figure}[!htb]
    \centering
    \begin{subfigure}{.99\textwidth}
      \centering
      \includegraphics[width=0.9\linewidth]{images/bicosine_hill/sequential/initial_mesh72x72.png}
      \label{fig:adv-rotating-bicosine-sequential}
    \end{subfigure}
    \caption{Initial condition for the bicosine hill in a rotating field problem.}
    \label{fig:adv-rotating-bicosine-hill-cn}
\end{figure}
\begin{figure}[!htb]
    \centering
    \begin{subfigure}{.99\textwidth}
      \centering
      \includegraphics[width=0.9\linewidth]{images/bicosine_hill/sequential/t=pi_mesh_30x30_nts_23_supg.png}
      \label{fig:adv-rotating-bicosine-sequential}
    \end{subfigure}
    \caption{Sequential solution using Crank-Nicolson upto $t = \pi$. The mesh is $30\times30$, with $23$ time steps. SUPG is used. The left image is of the 2D contour of the solution at time $t=\pi$. The right figure is plotted on a line passing through the center of the hill in a direction coinciding with the local advection velocity.}
    \label{fig:adv-rotating-bicosine-hill-cn}
\end{figure}

\begin{figure}[!htb]
    \centering
    \begin{subfigure}{.6\textwidth}
      \centering
      \includegraphics[width=0.9\linewidth]{images/bicosine_hill/space-time/t=pi_mesh_30x30x23_gls_+_supg_in_time_iso_u=0point5.png}
      \caption{}
      \label{fig:adv-rotating-bicosine-spacetime}
    \end{subfigure}
    % \\
    % \begin{subfigure}{.99\textwidth}
    %   \centering
    %   \includegraphics[width=0.9\linewidth]{images/bicosine_hill/space-time/t=pi_mesh_30x30x23_gls_+_supg_in_time_slice_and_plot.png}
    %   \caption{With stabilization. Both the overshoot and undershoot is much less than the unstabilized counterpart. The fluctuations are not diminished because the mesh resolution is very coarse at $30\times30$}
    %   \label{fig:adv-rotating-bicosine-nostab}
    % \end{subfigure}
    \caption{Space-time solution to the 2D bicosine-hill problem. Again the domain is the same $[0,1]^2$ and $t\in[0,\pi]$. The space-time mesh is $30\times30\times23$, i.e., the spatial discretization is $30\times30$ and 23 elements in the time direction. GLS is used for the spatial advection. I have used the Talyfem implementation of the SUPG for the time derivative}
    \label{fig:adv-rotating-bicosine-hill-cn}
\end{figure}

==> extras/6_16_comparison_sequential_2x.tex <==
\begin{figure}[!htb]
    \centering
    \begin{subfigure}{0.49\textwidth}
      \centering
      \includegraphics[width=0.9\linewidth]{images/bicosine_hill/sequential/k=1e-5_t=pi_mesh100x100_nts300_vel-times-2_tecplot2d.png}
      \label{fig:adv-rotating-bicosine-sequential}
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
      \centering
      \includegraphics[width=0.9\linewidth]{images/bicosine_hill/sequential/k=1e-5_t=pi_mesh100x100_nts300_vel-times-2_tecplot3d.png}
      \label{fig:adv-rotating-bicosine-sequential}
    \end{subfigure}
    \caption{Sequential solution using $100\times100$ mesh and 300 time steps. A small amount of undershoot can be noted.}
    \label{fig:bicosine-seq-vel-times-2-fine-mesh-sol}
\end{figure}

\begin{figure}[!htb]
    \centering
    \begin{subfigure}{0.49\textwidth}
      \centering
      \includegraphics[width=0.9\linewidth]{images/bicosine_hill/sequential/k=1e-5_t=pi_mesh72x72_nts72_vel-times-2_tecplot2d.png}
      \caption{$dt = \pi/72, u_{max} = 0.776, u_{min} = -0.26$}
      \label{fig:adv-rotating-bicosine-sequential}
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
      \centering
      \includegraphics[width=0.9\linewidth]{images/bicosine_hill/sequential/k=1e-5_t=pi_mesh72x72_nts150_vel-times-2_tecplot2d.png}
      \caption{$dt = \pi/150, u_{max} = 0.872, u_{min} = -0.066$}
      \label{fig:adv-rotating-bicosine-sequential}
    \end{subfigure}
    \caption{Sequential solution using $72\times72$ mesh. }
    \label{fig:bicosine-seq-vel-times-2-fine-mesh-sol}
\end{figure}

\begin{figure}[!htb]
    \centering
    \begin{subfigure}{0.7\textwidth}
      \centering
      \includegraphics[width=0.9\linewidth]{images/bicosine_hill/space-time/t=pi_k=1e-5_vel-times-2_mesh_72x72x72_stab_all_iso_u=0point77.png}
      \caption{$Mesh=72\times72\times72, u_{max} = 0.781, u_{min} = -0.042$}
      \label{fig:adv-rotating-bicosine-sequential}
    \end{subfigure}
    \begin{subfigure}{0.7\textwidth}
      \centering
      \includegraphics[width=0.9\linewidth]{images/bicosine_hill/space-time/t=pi_k=1e-5_vel-times-2_mesh_72x72x150_stab_all_iso_u=0point91.png}
      \caption{$Mesh=72\times72\times150, u_{max} = 0.919, u_{min} = -0.0164$}
      \label{fig:adv-rotating-bicosine-sequential}
    \end{subfigure}
    \caption{Spacetime solution with GLS stabilization (all terms)}
    \label{fig:bicosine-seq-vel-times-2-fine-mesh-sol}
\end{figure}

==> extras/6_17_comparison_sequential_5x.tex <==
\begin{figure}[!htb]
    \begin{subfigure}{0.49\textwidth}
      \centering
      \includegraphics[width=0.9\linewidth]{images/bicosine_hill/sequential/k=1e-5_t=0_mesh72x72_nts72_vel-times-5_tecplot3d.png}
      \caption{Initial condition}
      \label{fig:adv-rotating-bicosine-sequential}
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
      \centering
      \includegraphics[width=0.9\linewidth]{images/bicosine_hill/sequential/k=1e-5_t=pi_mesh72x72_nts72_vel-times-5.png}
      \caption{$t=\pi$}
      \label{fig:adv-rotating-bicosine-sequential}
    \end{subfigure}
    \caption{Sequential solution by Crank-Nicolson with stabilization. Mesh $72\times72$. Number of time step = 72. The Courant number $C$ is more than 3. The solution is absurd. We definitely need a finer mesh to capture the solution properly.}
    \label{fig:adv-rotating-bicosine-hill-cn}
\end{figure}

\begin{figure}[!htb]
    \centering
    \begin{subfigure}{0.99\textwidth}
      \centering
      \includegraphics[width=0.5\linewidth]{images/bicosine_hill/space-time/t=pi_mesh_72x72x72_gls_+_supg_in_time_iso_u=0point385_vel-times-5.png}
      \label{fig:adv-rotating-bicosine-sequential}
    \end{subfigure}
    \caption{Space-time solution. GLS stabilization is used. Showing the iso-surface of $u=0.385$. Visibly the thickness of the iso-surface decreases which should not happen. A finer mesh is needed for this high-velocity field. The solution is not fully correct but much better than the sequential solution.}
    \label{fig:adv-rotating-bicosine-hill-cn}
\end{figure}

==> extras/6_18_comparison_sequential_pure_advec.tex <==
\begin{figure}[!htb]
    \centering
    \begin{subfigure}{0.8\textwidth}
      \centering
      \includegraphics[width=0.9\linewidth]{images/bicosine_hill/sequential/t=pi_k=0_mesh_72x72_nts_72_supg_initial_final_compare.png}
      \label{fig:adv-rotating-bicosine-sequential}
    \end{subfigure}
    \caption{Sequential solution: Showing the hill height for the initial condition as well as the final time $t=\pi$. The diffusivity $\nu = 0$, that makes it a pure advective problem. Using Crank-Nicolson. The mesh is $72\times72$, with $72$ time steps. SUPG is used. The undershoot is not negligible. The peak height reduction is negligible.}
    \label{fig:adv-rotating-bicosine-hill-cn}
\end{figure}
\begin{figure}[!htb]
    \centering
    \begin{subfigure}{.8\textwidth}
      \centering
      \includegraphics[width=0.9\linewidth]{images/bicosine_hill/space-time/t=pi_mesh_72x72x72_k=0_gls_+_supg_in_time_peak_comparison.png}
      \label{fig:adv-rotating-bicosine-sequential}
    \end{subfigure}
    \caption{Space-time solution: Showing the hill height for the initial condition as well as the final time $t=\pi$. The diffusivity $\nu = 0$, that makes it a pure advective problem. Using Crank-Nicolson. The mesh is $72\times72\times72$. SUPG is used. There is a very small amount of undershoot. Also the reduction in the peak height is negligible.}
    \label{fig:adv-rotating-bicosine-hill-cn}
\end{figure}

==> extras/6_25_adref_pure_adv.tex <==
\begin{figure}
\centering
\begin{minipage}{.52\textwidth}
\includegraphics[width=0.99\linewidth]{results_data/1_adv_diff/pure_adv_threshold_surface.png}
\subcaption{The solution contour}
\end{minipage}%
\hskip 5pt
\begin{minipage}{.46\textwidth}
\includegraphics[width=0.99\linewidth]{results_data/1_adv_diff/pure_adv_final_mesh.png}
\subcaption{The mesh at the final refinement level}
\end{minipage}
\caption{Space-time solution contour of a bi-cosine cone in a rotating field}
\end{figure}


\begin{figure}[h!]
  \begin{center}
    \begin{tikzpicture}
      \begin{axis}[
          width=0.75\linewidth, % Scale the plot to \linewidth
          %grid=major, % Display a grid
          %grid style={line width=.1pt, draw=gray!50}, % Set the style
          xlabel=$s$, % Set the labels
          ylabel=$u$,
          legend style={at={(0.8,0.9)},anchor=north,legend columns=1}, % Put the legend below the plot
          x tick label style={rotate=0,anchor=north} % Display labels sideways
        ]
        \addplot+ [color=blue,mark=none]
        table[x expr={\thisrow{Points}},y expr={\thisrow{u}},col sep=space]{results_data/1_adv_diff/initial_condition_plot_over_line.txt}; 
        \addplot+ [color=red,thick, mark=none]
        table[x expr={\thisrow{Points}},y expr={\thisrow{u}},col sep=space]{results_data/1_adv_diff/final_time_plot_over_line.txt}; 
        \legend{ $t=0$, $t=1$}
      \end{axis}
    \end{tikzpicture}
    \caption{An overlay plot of the contour of the solution on a line passing through the center of the pulse, shown for the initial time and the final time. The peak height is intact, although there is a slight undershoot as well as ``thickening" of the pulse at the bottom. $s$ is the length parameter on the line.}
  \end{center}
\end{figure}

==> extras/6_50_error_conv_comparison.tex <==



\begin{figure}
\centering
\begin{minipage}{.49\textwidth}
  \begin{center}
  \begin{tikzpicture}
      \begin{loglogaxis}[
    %   xmode=log,
    %   ymode=log,
    %   log ticks with fixed point,
          width=0.99\linewidth, % Scale the plot to \linewidth
          xlabel=$\textsc{\# DOF}$, % Set the labels
          legend style={at={(0.75,0.92)},anchor=north,legend columns=1}, % Put the legend below the plot
          x tick label style={rotate=0,anchor=north}
        ]
        \addplot 
        table[x expr={(\thisrow{nodes})},y expr={\thisrow{eta}},col sep=space]{results_data/2_diff/uniform_refinement_3_to_6.txt};
        \addplot 
        table[x expr={(\thisrow{nodes})},y expr={\thisrow{eta}},col sep=space]{results_data/2_diff/adref_lev_3_plus_3.txt};
        \legend{Uniform, Adaptive}
      \end{loglogaxis}
    \end{tikzpicture}
    \subcaption{Convergence of $\normL{\eta}{\Omega}$}
    \label{fig:eta-conv-diffusion-compare-uniform-adref}
    \end{center}
\end{minipage}
\hskip 5pt
\begin{minipage}{.49\textwidth}
  \centering
  \begin{tikzpicture}
      \begin{loglogaxis}[
          width=0.99\linewidth, % Scale the plot to \linewidth
          %grid=major, % Display a grid
          %grid style={line width=.1pt, draw=gray!50}, % Set the style
          xlabel=$\textsc{\# DOF}$, % Set the labels
          %ylabel=$\eta_{\Omega}$,
          legend style={at={(0.75,0.92)},anchor=north,legend columns=1}, % Put the legend below the plot
          x tick label style={rotate=0,anchor=north} % Display labels sideways
        ]
        \addplot 
        table[x expr={(\thisrow{nodes})},y expr={\thisrow{L2_Err}},col sep=space]{results_data/2_diff/uniform_refinement_3_to_6.txt};
        \addplot 
        table[x expr={(\thisrow{nodes})},y expr={\thisrow{L2_Err}},col sep=space]{results_data/2_diff/adref_lev_3_plus_3.txt};
        \legend{Uniform, Adaptive}
      \end{loglogaxis}
    \end{tikzpicture}
    \subcaption{Convergence of $\normL{v-\vh}{\Omega}$}
    \label{fig:eL2-conv-diffusion-compare-uniform-adref}
\end{minipage}
\caption{Comparison of the error indicator and the error in $L^2$-norm in both uniform and adaptive refinement}
\end{figure}



==> extras/6_51_error_conv_adaptive.tex <==
\begin{figure}
\centering
\begin{minipage}{.49\textwidth}
  \begin{center}
  \begin{tikzpicture}
      \begin{loglogaxis}[
    %   xmode=log,
    %   ymode=log,
    %   log ticks with fixed point,
          width=0.99\linewidth, % Scale the plot to \linewidth
          xlabel=$\textsc{\# DOF}$, % Set the labels
          legend style={at={(0.75,0.92)},anchor=north,legend columns=1}, % Put the legend below the plot
          x tick label style={rotate=0,anchor=north}
        ]
        \addplot 
        table[x expr={\thisrow{nodes}},y expr={\thisrow{eta}},col sep=space]{results_data/2_diff/Statistics_k_1e-4.txt};
        \addplot 
        table[x expr={\thisrow{nodes}},y expr={\thisrow{L2_Err}},col sep=space]{results_data/2_diff/Statistics_k_1e-4.txt}; 
        \legend{\small $\eta_{\Omega}$, $\|e\|_{L^2(\Omega)}$}
      \end{loglogaxis}
    \end{tikzpicture}
    \subcaption{$\|e\|_{L^2(\Omega)}$ and $\eta_{\Omega}$ \\behavior for the diffusion problem}
    \label{fig:eta-conv-diffusion}
    \end{center}
\end{minipage}%
\hskip 5pt
\begin{minipage}{.49\textwidth}
  \centering
  \begin{tikzpicture}
      \begin{loglogaxis}[
          width=0.99\linewidth, % Scale the plot to \linewidth
          %grid=major, % Display a grid
          %grid style={line width=.1pt, draw=gray!50}, % Set the style
          xlabel=$\textsc{\# DOF}$, % Set the labels
          %ylabel=$\eta_{\Omega}$,
          legend style={at={(0.75,0.92)},anchor=north,legend columns=1}, % Put the legend below the plot
          x tick label style={rotate=0,anchor=north} % Display labels sideways
        ]
        \addplot 
        table[x expr={\thisrow{nodes}},y expr={\thisrow{eta}},col sep=space]{results_data/1_adv_diff/Statistics_k_0000.txt}; 
        \addplot 
        table[x expr={\thisrow{nodes}},y expr={\thisrow{eta}},col sep=space]{results_data/1_adv_diff/Statistics_k_1e-1.txt}; 
        \legend{ $\kappa=0$, $\kappa=10^{-1}$}
      \end{loglogaxis}
    \end{tikzpicture}
    \subcaption{Overall estimator behavior for the advection-diffusion problem}
    \label{fig:eta-conv-adv-diff}
\end{minipage}
\caption{Convergence of the error indicator and with the error norm in an adaptive refinement case}
\end{figure}

==> extras/7_01_gmres_conv.tex <==
\begin{table}[]
\centering
\begin{tabular}{ccccccc}
\hline
\multirow{2}{*}{} & \multicolumn{6}{c}{No stabilization}                                                                 \\ \cline{2-7} 
                  & \multicolumn{3}{c|}{No preconditioner}                   & \multicolumn{3}{c}{Jacobi preconditioner} \\ \hline
                  & Time & \# iter     & \multicolumn{1}{c|}{$\|e\|_{L^2}$} & Time       & \# iter      & $\|e\|_{L^2}$  \\ \hline
$1$               & 396  & 0.000586028 & \multicolumn{1}{c|}{7.89639}       & 303        & 0.000585908  & 9.30753        \\
$1e-1$            & 1030 & 0.000100769 & \multicolumn{1}{c|}{19.4491}       & 367        & 0.000106855  & 11.3013        \\
$1e-2$            & 660  & 0.000240627 & \multicolumn{1}{c|}{12.9032}       & 71         & 0.000190887  & 2.22327        \\
$1e-3$            & 570  & 0.000135848 & \multicolumn{1}{c|}{10.6704}       & diverges   & -            & -              \\
$1e-5$            & 561  & 0.000165266 & \multicolumn{1}{c|}{10.9174}       & diverges   & -            & -              \\
$1e-7$            & 561  & 0.000169247 & \multicolumn{1}{c|}{11.1811}       & diverges   & -            & -              \\ \hline
\end{tabular}
\end{table}

\begin{table}[]
\centering
\begin{tabular}{ccccccc}
\hline
\multirow{2}{*}{} & \multicolumn{6}{c}{With GLS stabilization}                                                           \\ \cline{2-7} 
                  & \multicolumn{3}{c|}{No preconditioner}                   & \multicolumn{3}{c}{Jacobi preconditioner} \\ \hline
                  & Time & \# iter     & \multicolumn{1}{c|}{$\|e\|_{L^2}$} & Time    & \# iter        & $\|e\|_{L^2}$   \\
$1$               & 391  & 0.000633444 & \multicolumn{1}{c|}{7.5761}        & 299     & 0.000633343    & 9.25117         \\
$1e-1$            & 494  & 0.000100009 & \multicolumn{1}{c|}{9.30299}       & 291     & 9.84E-05       & 8.72568         \\
$1e-2$            & 282  & 0.000181836 & \multicolumn{1}{c|}{6.05571}       & 32      & 0.000163062    & 1.2298          \\
$1e-3$            & 316  & 0.000200764 & \multicolumn{1}{c|}{5.85373}       & 51      & 0.000198699    & 1.69914         \\
$1e-5$            & 317  & 0.000205731 & \multicolumn{1}{c|}{6.19172}       & 233     & 0.000200746    & 6.98957         \\
$1e-7$            & 317  & 0.000205814 & \multicolumn{1}{c|}{5.98}          & 239     & 0.000200762    & 8.19306         \\ \hline
\end{tabular}
\end{table}


==> extras/8_old_images.tex <==
\begin{figure}[!htb]
    \centering
    \begin{subfigure}{0.99\textwidth}
      \centering
      \includegraphics[width=0.99\linewidth]{images/refinement/conv_plot_case1.eps}
      %\label{fig:adv-rotating-bicosine-sequential}
    \end{subfigure}
    \caption{Log-log plot of the the overall estimator for the advection-diffusion problem}
    %\label{fig:adv-rotating-bicosine-hill-cn}
\end{figure}
\begin{figure}[!htb]
    \centering
    \begin{subfigure}{0.99\textwidth}
      \centering
      \includegraphics[width=0.99\linewidth]{images/refinement/conv_plot_case2.eps}
      %\label{fig:adv-rotating-bicosine-sequential}
    \end{subfigure}
    \caption{Log-log plot of the $L^2$-error and the overall estimator for the diffusion problem}
    %\label{fig:adv-rotating-bicosine-hill-cn}
\end{figure}


\begin{figure}[!htb]
    \centering
    \begin{subfigure}{0.99\textwidth}
      \centering
      \includegraphics[width=0.99\linewidth]{images/pure_advection/profile_comparison_t0_t1.png}
      %\label{fig:adv-rotating-bicosine-sequential}
    \end{subfigure}
    \caption{Profile comparison with space-time}
    %\label{fig:adv-rotating-bicosine-hill-cn}
\end{figure}
\begin{figure}[!htb]
    \centering
    \begin{subfigure}{0.99\textwidth}
      \centering
      \includegraphics[width=0.99\linewidth]{images/pure_advection/solution_comparison_CN_linearbasis_256x256_ts256.png}
      %\label{fig:adv-rotating-bicosine-sequential}
    \end{subfigure}
    \caption{Profile comparison with Crank-Nicolson}
    %\label{fig:adv-rotating-bicosine-hill-cn}
\end{figure}
\clearpage

\begin{figure}[!htb]
    \centering
    \begin{subfigure}{0.99\textwidth}
      \centering
      \includegraphics[width=0.99\linewidth]{images/refinement/bicosine_pulse_iso_vol.png}
      %\label{fig:adv-rotating-bicosine-sequential}
    \end{subfigure}
    \caption{Refined iso volume}
    %\label{fig:adv-rotating-bicosine-hill-cn}
\end{figure}
\begin{figure}[!htb]
    \centering
    \begin{subfigure}{0.99\textwidth}
      \centering
      \includegraphics[width=0.99\linewidth]{images/refinement/peak_comparison_case1.png}
      %\label{fig:adv-rotating-bicosine-sequential}
    \end{subfigure}
    \caption{Refined state}
    %\label{fig:adv-rotating-bicosine-hill-cn}
\end{figure}

==> sections/0_abstract.tex <==
% \documentclass[../main.tex]{subfiles}
% \begin{document}
We present a full space-time numerical solution of the advection-diffusion equation using a continuous Galerkin finite element method. The Galerkin/least-square method is employed to ensure stability of the discrete variational problem. In the full space-time formulation, time is considered another dimension, and the time derivative is interpreted as an additional advection term of the field variable. We derive \textit{a priori} error estimates and illustrate spatio-temporal convergence with several numerical examples. We also derive \textit{a posteriori} error estimates, which coupled with adaptive space-time mesh refinement provide efficient and accurate solutions. The accuracy of the space-time solutions is illustrated against analytical solutions as well as against numerical solutions using a conventional time-marching algorithm.
% \end{document}

==> sections/1_introduction.tex <==
% \documentclass[../main.tex]{subfiles}
% \begin{document}
\section{Introduction}\label{sec:introduction}

% In the context of solving time-dependent partial differential equations, the space-time finite element analysis refers to the paradigm where the solution to the PDE is obtained as a function of both space and time simultaneously without requiring any time-marching algorithm. In general, 
Numerically solving a transient (or evolution) problem characterized by a partial differential equation (PDE) requires that the continuous problem be discretized in space and time. The standard way to deal with this dual discretization, is to use a suitable time-marching algorithm coupled with some form of spatial discretization such as the finite difference method (FDM), the finite element method (FEM), the finite volume method (FVM) or the more recent isogeometric analysis (IgA). In some cases, the time marching algorithms themselves are based on finite difference methods and are used along with the above mentioned spatial discretizations.\footnote{In addition, in the case where FEM is used to discretize the space, the time-marching algorithm can also be based on finite elements. This formulation also known as \textit{space-time formulation} is usually applied to a single time step. This approach has been successfully applied to a rich variety of applications \cite{tezduyar1992newI,tezduyar1992newII,takizawa2012space}. The current paper, in contrast, explores solving for large space-time blocks.} Generally speaking, these approaches consider the spatio-temporal domain over which the solution is desired as a product of a spatial domain with a temporal domain, with independent discretization and analysis of each of these components.

% All these classes of discretization are well understood and popularly used in many areas. But this separation of space and time does lead to difficulty in effectively implementing adaptive refinement techniques. Moreover, when designing parallel algorithms for massively parallel supercomputers, these methods can pose severe scalability issues since the algorithms are essentially ``sequential". 

An alternative strategy to ``time-marching" is to  discretize and solve for the full ``space-time" domain together. Any combination of spatial and temporal discretization can be used -- for instance, finite difference schemes in both space and time; or FEM in space and FDM in time; or FEM in both space and time. In particular, in the context of FEM, this constitutes a second type of ``space-time" formulation, where finite element formulation is used in both space and time, but time marching is not employed. A major attraction for formulating a problem in space-time is the possibility of improved parallel performance. The idea of parallelism in both space and time builds on a rich history of parallel time integration~\cite{Hackbusch:1985:PMM:4673.4714, lubich1987multi, horton1995space}. We refer to \cite{gander201550,vandewalle2013parallel} for a review of such methods.


The finite element community has a history of considering solutions to time dependent PDEs in space-time. The earliest references to space-time formulations go back to the mid 1980's. Babuska and co-workers~\cite{babuska1989h,babuvs1990h} developed $h-p$ versions of finite element method in space along with p and $h-p$ versions of approximations in time for parabolic problems. Around the same time, Hughes and Hulbert formulated a space-time finite element method for elastodynamics problem \cite{hughes1988space} and general hyperbolic problems \cite{hulbert1990space} using time-discontinuous Galerkin method. Recently, there has been increasing interest in revisiting this problem given access to larger computational resources \cite{langer2016space, dyja2018parallel, ishii2019solving}. In this work, we tackle two key aspects associated with solving evolution equations in space-time -- stability and computational cost. We focus on a particular family of PDE's, specifically the time dependent advection-diffusion equation, with the time dependent diffusion equation as a special case (when the advection term goes to zero). 

%Schwab and Stevenson developed space-time adaptive wavelet methods using tensor-product wavelet bases for parabolic evolution problems \cite{schwab2009space}.

\textbf{Stability of the discrete space-time formulation}: When solving parabolic equations through space-time methods, the question of stability of the ensuing discrete system becomes important. As mentioned earlier, in a sequential setting, the time derivative term is treated separately during temporal discretization. But when the advection-diffusion equation is formulated in space-time (i.e. time is considered another dimension, like the rest of the spatial dimensions), the time evolution term (first order derivative with respect to time) can be mathematically seen as an ``advection in time dimension" term and can be grouped with the other spatial first derivatives in the equation \cite{bank2017arbitrary}. This identification is mathematically consistent since all the first order derivatives, irrespective of whether they are spatial or temporal, have a sense of ``directionality" attached to them (the actual direction is determined by the sign of their coefficients). Mathematically then, the problem can be seen as a ``generalized advection-diffusion equation" in space-time, except, there is no diffusion term associated with the time dimension. This type of equation, when solved through the standard Galerkin method, can suffer from a lack of stability and end up with spurious oscillations \cite{brooks1982streamline, donea2003finite}. Andreev and Mollet \cite{andreev2012stability, mollet2014stability} analyzed the stability of space-time FEM discretizations of abstract linear parabolic evolution equations. Steinbach \cite{steinbach2015space} also analyzed the stability of the heat equation in space-time setting and derived error bounds using unstructured space-time finite elements. In 2017, Langer et al. \cite{langer2016space} used a time-upwind type Petrov-Galerkin basis function similar to the streamline diffusion method, to solve the heat equation in space-time moving domains. There is a large body of literature available that deals with treating non self-adjoint operators through finite element method \cite{brooks1982streamline,johnson1984finite,johnson1986streamline,hughes1989new,hughes1995multiscale}, a review of which can be found in \cite{franca2004stabilized}. In this work, we build upon this body of work and ensure stability of the discrete variational form by using a Galerkin/least squares (GLS) approach \cite{hughes1989new, franca1992stabilized}. We show that GLS provides stability to the discrete space-time problem and derive \textit{a priori} error bounds in the discrete norm associated with the bilinear form.

% the geometric domain with finite elements to interpolate the unknown field variables. But the variation of the solution with time is not expressed through the Lagrangian basis function, rather, a finite difference approach is applied in most cases. This technique is generally known as time-stepping method, where the entire time duration is divided into a number of steps and each step is solved sequentially. On the other hand, space-time finite element analysis provides an alternative to this paradigm, where the solution for the whole spacetime domain is solved together. Thus the final solution is the solution for the whole space-time domain, and not just the solution for the final time. A few of the relevant texts are \cite{steinbach2015space}, \cite{langer2016space}, \cite{hughes1988space}, \cite{dyja2018parallel} etc.

% Accommodating the time dimension as another dimension within the FEM problem brings with it a whole range of  possibilities that can be exploited to design computational methodologies that can scale to leverage the availability of very large computing resources. In particular, space-time analysis paradigm creates opportunity for parallelism in a wider sense than the more conventional sequential approach. This is because, in this type of analysis, the parallelism can be applied in both space and time, rather than either one of them at a time. This also opens up the opportunity of adaptive mesh refinement in both space and time, rather than refining only a space domain at a particular time mark. For problems where the field variable(s) naturally exhibit high gradients in both space and time, the refinement in a "space-time" region becomes a natural choice. 

% Galerkin least squares method was introduced by Hughes et al. ~\cite{hughes1989new} in 1989 to solve advective diffusive equations through finite element method.

% \begin{itemize}
%     \item Evolution problems
%     \item Intro to time-parallelism
%     \item Solving parabolic problem in FE with time as another dimension
%     \item Bloated degrees of freedom: adaptive refinement
% \end{itemize}
%formulate the time dependent advection diffusion equation through a space-time finite element framework. To overcome this, we use th
\textbf{Reducing computational cost via space-time adaptivity}: A space-time formulation adds one more dimension to concurrently discretize. A 2D problem needs a 3D mesh and a 3D problem needs a 4D mesh. Thus the number of degrees of freedom in the resulting linear system can become significantly larger than the corresponding sequential problem. %From the computational point of view, this means that the memory requirements can be  high. 
Prior research has shown that this increased computational cost is ideally suited to sustained parallelism \cite{horton1995space,farhat2003time,cortial2009time,friedhoff2012multigrid,emmett2012toward,speck2012massively,langer2016space,dyja2018parallel,ishii2019solving}. Additional efficiencies can be accessed by making efficient use of adaptive mesh refinement (AMR) in space-time \cite{abedi2004spacetime,dyja2018parallel,ishii2019solving,christopher2020parallel,gomez2023design}. To this end, we mathematically derive a residual-based \textit{a posteriori} error indicator which can be used to estimate elementwise errors. This enables us to leverage the benefits of AMR in a space-time setting which render very accurate solution to the diffusion problem and the advection-diffusion problems considered here. 
% This adaptive refinement strategy in space-time is very different in nature compared to an adaptive refinement in a sequentially driven time-marching algorithm. In a sequential setting, the refinement in the next step is somewhat ``predetermined" from the current time-step. But in a space-time domain the \textit{a posteriori} error calculation is more natural.

The rest of the content of this paper is organized as follows. In \secref{sec:math-formulation}, we introduce the mathematical formulation of the problem. We formulate the continuous and the discrete problems and state the relevant function spaces. We then prove the stability of the discrete bilinear form and then derive \textit{a priori} and \textit{a posteriori} error estimates. Then in \secref{sec:numerical-examples}, we present numerical examples that validate the theoretical results of \secref{sec:math-formulation}, and also demonstrate the advantages of using adaptive mesh refinement in space-time analysis. Finally in \secref{sec:conclusion}, we draw conclusions and make some comments about future research directions.



% \end{document}

==> sections/2_math_gls.tex <==
% \documentclass[../main.tex]{subfiles}
% \begin{document}
\section{Mathematical Formulation}\label{sec:math-formulation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The time-dependent linear advection-diffusion equation}\label{subsec:pde}
\begin{figure}[!t]
	\centering
	\def \mpagefrac{0.7}
	\begin{minipage}{\mpagefrac\textwidth}
		\centering
		\begin{tikzpicture}
		\def \myscale{\mpagefrac / 0.5} % needs \usepackage{calc}
		\draw (0, 0) node[inner sep=0] {\includegraphics[trim=3.3in 0.5in 3.3in 0.8in, clip,width=0.7\linewidth]{images/domain-notations.pdf}};
		\draw (0, 0) node {$ \stDom = \spDom \times \temporalInterval $};
		\draw (-2.5*\myscale, 3.0*\myscale) node {$t$};
		\draw (-2.7*\myscale,  2.1*\myscale) node {$t=T$};
		\draw (-2.7*\myscale, -1.5*\myscale) node {$t=0$};
		\draw (-2.2*\myscale, -2.7*\myscale) node {$x_1$};
		\draw ( 2.6*\myscale, -1.5*\myscale) node {$x_2$};
		\draw[stealth-, thick] (-0.2*\myscale, -1.6*\myscale) -- ++(0.5*\myscale,-1.3*\myscale) node[right, black, fill=white, anchor=north]{$\bit = \spDom\times \{0\}$};
		\draw[stealth-, thick] (-0.2*\myscale, 2.1*\myscale) -- ++(0.2*\myscale,1.0*\myscale) node[right, black, fill=white, anchor=south]{$\bft = \spDom\times \{T\}$};
		\draw[stealth-, thick] (1.45*\myscale, 0.1*\myscale) -- ++(0.7*\myscale,1.0*\myscale) node[right, black, fill=white, anchor=south west]{$\bsp = \partial \spDom \times (0,T)$};
		%		\draw (3*\myscale, 3*\myscale) node {$ (3, 3) $};
		%		\draw (-3*\myscale, -3*\myscale) node {$ (-3, -3) $};
		\end{tikzpicture}
	\end{minipage}
	\caption{Schematic depiction of the space-time domain $ \stDom = \spDom \times \temporalInterval $, where $ \spDom \subset \mathbb{R}^{\nsd} $, and $ \temporalInterval = [0,T] \subset \mathbb{R}^{+}. $} 
	\label{fig:schematic-space-time-domain}
\end{figure}
Consider a bounded spatial domain $\spDom \in \mathbb{R}^{\nsd}, \nsd=1,2,3$ with Lipschitz continuous boundary $\partial \spDom$ and a bounded time interval $\temporalInterval = (0,T] \in \mathbb{R^+}$. We define the space-time domain as the Cartesian product of the two as $\stDom = \spDom \times \temporalInterval = \spDom\times(0,T]$ (see \figref{fig:schematic-space-time-domain}). The overall boundary of this space-time domain is defined as $\Gamma = \partial \stDom$. This overall boundary is the union of the spatial boundaries and the time boundaries. The spatial domain boundary is denoted by $\bsp = \partial \spDom \times (0,T]$; whereas the time boundaries are denoted by $\Gamma_{_0} = \bar{\spDom}\times\{0\}$ and $\Gamma_{_T} = \bar{\spDom}\times\{T\}$ which are the initial and final time boundaries respectively. The closure of the space-time domain is $ \bar{\stDom} = \stDom \cup \bsp \cup \Gamma_{_0} $. The advection-diffusion equation can then be written for the scalar function $u: \stDom \rightarrow \mathbb{R}$ as:
\begin{subequations}\label{pde:linear-advection-diffusion}
\begin{align}
    \ut + \adiv u- \visco \laplacian u &=f \quad \textrm{in}\quad\stDom\label{pde:linear-advection-diffusion-equation},\\
u&=g\quad \textrm{on}\quad\bsp\label{pde:linear-advection-diffusion-BC},\\
u(\cdot,t=0)&=u_0\quad \textrm{on}\quad \Gamma_{0},\label{pde:linear-advection-diffusion-IC}
\end{align}
\end{subequations}
with
%\begin{align}\label{operator:pde-abstract-operator-full}
%    \opLT u = \ut + \adv\cdot\grad u- \grad\cdot(\visco\grad u),
%\end{align}
where $f: \stDom \rightarrow \mathbb{R}$ is a smooth forcing function,  $\visco >0 $ is the diffusivity and does not depend on $u$; and Dirichlet boundary conditions are imposed on the boundary $\bsp$. Note that $\grad$ is the usual gradient operator in the space $\mathbb{R}^{\nsd}$, i.e., $ \grad \equiv (\nicefrac{\partial}{\partial x}, \nicefrac{\partial}{\partial y}) $ for $ \nsd = 2 $ and $ \grad \equiv (\nicefrac{\partial}{\partial x}, \nicefrac{\partial}{\partial y}, \nicefrac{\partial}{\partial z}) $ for $ \nsd = 3 $ respectively. We further define the space-time gradient operator $\gradst$ as: $ \gradst \equiv (\grad, \nicefrac{\partial}{\partial t}) $.

Let us define two operators $ \opL $ and $ \opLT $ as follows:
\begin{subequations}
	\begin{align*}
	\opL u &= \adiv u- \visco \laplacian u, \\
	\text{and}\ \ \opLT u &= \ut + \opL \\
	&= \ut + \adiv u- \visco \laplacian u.
	\end{align*}
\end{subequations}

Since $ \visco > 0$, therefore $ \opL $ is elliptic and it follows that the operator $\opLT = (\nicefrac{\partial}{\partial t} + L)$ is strictly parabolic. Such equations are typically solved with a \textit{method of lines} discretization, by solving a series of discrete equations sequentially. At each ``time-step'', the solution is assumed to be a function of the spatial variables only. In the context of the Galerkin methods, this spatial approximation takes the form of a (discrete) Sobolev space, e.g., the solution at the $ i^{\text{th}} $ step, $ u^i(x) \in  H^1(\spDom) $. But in this work, our focus will be \textit{coupled space-time} formulation of the advection-diffusion equation where we approximate the solution in a Sobolev space defined on the full space-time domain (i.e., $ u(x,t) \in H^1(\stDom) $). As alluded to in the introduction, this kind of problem formulation requires some form of stabilization. Here, the Galerkin/Least Squares method is used for this purpose.

When we add such stabilizing terms to the original variational problem, we essentially end up adding some numerical ``diffusion" into the system. More importantly, diffusion may be introduced in the time direction as well, which is absent in the original parabolic equation. We show, in the results section, that careful design of stabilization ensures that this diffusion in the time direction can be made arbitrarily small. In essence, then, the equation becomes elliptic in the space-time domain. Anticipating such changes to the equation, we can cast this parabolic equation as a generalized elliptic equation as follows,
% And when we try to solve this problem through the Galerkin/Least squares method, we add some higher order derivative terms with respect to time. 
\begin{align}\label{pde:generalized-elliptic-summation-form}
    -\Xsum_{i=1}^{\nsd+1}\Xsum_{j=1}^{\nsd+1} \frac{\partial}{\partial x_i}\left( \ellipticA_{ij} (x) \frac{\partial u}{\partial x_j}\right) + \Xsum_{i=1}^{\nsd+1} \ellipticB_i(x)\frac{\partial u}{\partial x_i} = f,
\end{align}
where $\ellipticA_{ij}$ and $\ellipticB_i$ are the components of $\ellipticAmat\in \mathbb{R}^{(\nsd+1)\times(\nsd+1)}$ and $\ellipticBvec\in \mathbb{R}^{(\nsd+1)}$:
\begin{align} \label{expr:ellipticity-matrix-original}
  \ellipticAmat=
    \begin{bmatrix}
    \visco & 0 & 0 & 0 \\
     0 & \visco & 0 & 0\\
     0 & 0 & \visco & 0 \\
     0 & 0 & 0 & 0
    \end{bmatrix}
    ,\qquad
    \ellipticBvec = 
    \begin{bmatrix}
    b_1\\b_2\\ b_3\\ 1
    \end{bmatrix},
\end{align}
where all off-diagonal entries as well as the last diagonal entry in $\mmat{A}$ are zero.
% Note that the last diagonal entry is zero as well, which is because the original equation doesn't have any second derivative with respect to time.
After we finish the formulation with Galerkin/Least squares, we will eventually have a small positive real entry in the last diagonal term along with some non-zero terms in the off-diagonals. Note that we have also assumed an isotropic diffusive medium, so the principal diffusivity values are the same in all directions. This assumption can be trivially relaxed. In the $\adv$ vector, along with the spatial advection components, we have the ``advection in time" component which has the value 1.

This equation can then be rewritten in a more compact form:
\begin{align}\label{pde:generalized-elliptic-operator-form}
    \left(-\gradst\cdot\ellipticAmat\cdot\gradst + \ellipticBvec\cdot\gradst\right)u = f.
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Variational problem and function spaces}\label{subsec:var-prob-function-spaces}
Let us define the function space $V$ as 
\begin{align}\label{def:function-space-V}
V = \{v\in H^1(\stDom) : v = 0 \textrm{ on }\bit \cup \bsp \},
\end{align}
the $ L^2 $-inner product and $ L^2 $-norm in the space-time domain $ \stDom $ as
\begin{align*}
(v,w) &= \int_{\stDom} vw \text{ } d\stDom = \int_{0}^{T}\int_{\spDom} vw \text{ } d\spDom dt, \\
\norm{u} &= \sqrt{\inner{u}{u}}.
\end{align*}
On any $ \Gamma \subset \partial \stDom $, we define the $ L^2 $-inner product and norm by using a subscript:, e.g.,
\begin{align*}
(v,w)_{\Gamma} = \int_{\Gamma} vw \ d\Gamma \quad \text{and} \quad \norm{u}_{\Gamma} = \sqrt{\inner{u}{u}_{\Gamma}}.
\end{align*}
A special case is the integration over the final time boundary $ \bft $, for which we will use:
\begin{align*}
(v,w)_{\bft} = \int_{\spDom} v(\xvec,T) \ w(\xvec,T) \ d\spDom \quad \text{and} \quad \norm{u}_{\bft} = \sqrt{\inner{u}{u}_{\bft}}.
\end{align*}
Unless otherwise stated, an inner product or a norm without any subscript will be assumed  to be that calculated in $ \stDom $. A typical integration-by-parts in the \textit{spatial dimensions} can be written as:
\begin{align}
\inner{v}{\laplacian w} = \intTimeSpace v\laplacian w \ d\spDom \ dt &= \intTime \left[ -\intSpace \grad v \cdot \grad w\ d\spDom + \int_{S=\partial \spDom} v (\normalvec\cdot\grad w) \ dS \right]dt \\
&= -\inner{\grad v}{\grad w} + \inner{v}{\normalvec\cdot \grad w}_{\bsp}.
\end{align}
This expression looks identical to the formula when the inner product is defined in just the spatial dimensions.

If $\ustar(\mvec{x},t)$ is the exact solution of equation \eqref{pde:linear-advection-diffusion}, then $ \ustar $ can be written as
\begin{align}\label{exact-sol-decomposition}
    \ustar(\mvec{x},t) &= u(\mvec{x},t)+h(\mvec{x},t),
\end{align}
where $ u \in \spaceV $, and $ h \in H^1(\stDom) $ is some known function such that $ h|_{\bsp} = g $ and $ h|_{\bit} = u_0 $.
%\begin{align}\label{def:v}
%    v(\mvec{x},t) &= 0, \text{ when } \mvec{x}\in\bsp\cup\Gamma_{_0}
%\end{align}
%and $g$ is some function in $V$ with the property:
%\begin{align}\label{def:g}
%    g(\mvec{x},t) &= 
%    \begin{cases}
%    u_0(\mvec{x}), & \text{ when } \mvec{x}\in\Gamma_{_0}\\
%    0, & \text{ when } \mvec{x}\in\bsp.
%    \end{cases}
%\end{align}
Substituting \eqref{exact-sol-decomposition} into \eqref{pde:linear-advection-diffusion-equation}, we have $\opLT u = f - \opLT h$. By defining the new right hand side as $F = f - \opLT h$, we can recast \eqref{pde:linear-advection-diffusion} as
\begin{subequations}\label{pde-mod:linear-advection-diffusion}
\begin{align}
    \opLT u &=F\quad \textrm{in}\quad\stDom\label{pde-mod:linear-advection-diffusion-equation}\\
    u &=0 \quad \textrm{on}\quad\bsp\label{pde-mod:linear-advection-diffusion-BC}\\
    u(\mvec{x},t_0) &= 0\quad \textrm{on}\quad \Gamma_{0}. \label{pde-mod:linear-advection-diffusion-IC}
\end{align}
\end{subequations}


We also define the following function space of bounded divergence-free convection fields:
\begin{align}
\spaceVdiv = \setbuilder{v \in \mvec{W}^{1,\infty} :\ \divergence v = 0\ \text{in}\ \stDom},
\end{align}
where $ \mvec{W}^{1,\infty} = [W^{1,\infty}]^{\nsd} $ is a product function spaces. Given $ \adv \in \spaceVdiv $ and $ F\in L^2(\stDom) $, the variational problem for \eqref{pde-mod:linear-advection-diffusion} is then to find $u \in V$ such that
\begin{equation}\label{var-prob:continuous-variational-form}
    \bform(u,v) = l(v)\quad \forall v \in V,
\end{equation}
where
\begin{subequations}\label{def:continuous-bilinear-linear-forms}
\begin{align}
    \bform(u,v) &= (u_t,v) + (\adv\cdot\grad u, v) + (\visco\grad u, \grad v), \label{def:continuous-bilinear-form}\\
    l(v) &= (F,v). \label{def:continuous-linear-form}
\end{align}
\end{subequations}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Discrete variational problem}\label{subsec:discrete-variational-problem}
Define $\mesh$ as the partition of $\stDom$ into a finite number of non-overlapping elements. For the finite element problem, we define the finite dimensional subspace $V_h \subset V$ as
\begin{align}\label{def:functiona-space-Vh}
    V_h = \{\vh \in V: \vh|_K \in P_m(K), K \in \mesh \},
\end{align}
where $P_m(K)$ is the space of polynomial functions of degree less than or equal to $m$ in $K$. We also define the discrete inner product on this mesh as
\begin{align} \label{def:discrete-norm}
\innerh{u}{v} = \Xsum_{K \in \mesh} \int_{K} uv \ dK,
\end{align}
and the associated discrete norm as
\begin{align}
\normh{\uh} = \sqrt{\innerh{\uh}{\uh}}.
\end{align}
Given $ \adv\in \spaceVdiv $ and $ F\in L^2(\stDom) $, the discrete counterpart of \eqref{var-prob:continuous-variational-form} is then to find $ \uh \in \spaceVh $ such that
\begin{equation}\label{var-prob:discrete-variational-form}
\bform(\uh, \vh) = l(\vh)\quad \forall \vh \in \spaceVh.
\end{equation}

Solutions to equation \eqref{var-prob:discrete-variational-form} can exhibit numerical instabilities because the bilinear form $\bform(u=\uh,\vh)$ in equation \eqref{var-prob:discrete-variational-form} is not strongly coercive in $\spaceVh$ \cite{larson2013finite,langer2016space}. This issue can be tackled by adding some amount of numerical diffusion in the time direction or by adding upwind type correction to the weighting functions ~\cite{langer2016space,  steinbach2015space}. %But as can be expected, the difficulty increases when advection is present in the system. 
In what follows, we try to establish a stable variational form of the space-time advection-diffusion problem stated in \eqref{pde-mod:linear-advection-diffusion} by applying the Galerkin/least square (GLS) method. The resulting discrete problem is stable and converges to the original PDE in the limit of the mesh size approaching zero.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Stabilization through Galerkin Least Squares}\label{sec:galerkin-least-squares}

% \subsection{Weak Form}\label{subsec:gls-weak-form}
An equation of the form $\opLT u=F$ can be cast into a least square minimization problem as
\begin{align}\label{eq:least-square-minimization}
    \uh = \argmin_{v\in \spaceVh} \| \opLT v-F \|^2.
\end{align}
The resulting Euler-Lagrange equation corresponding to this minimization problem is
\begin{align}\label{eq:least-square-euler-lagrange}
    \innerh{\opLT \uh}{\opLT \vh} = \innerh{F}{\opLT \vh}.
\end{align}
In the GLS formulation, equation \eqref{eq:least-square-euler-lagrange} is added to equation \eqref{var-prob:continuous-variational-form} (specifically, its discrete counterpart), i.e., we seek $\uh \in V_h$ such that,
% \begin{align}
%     (\opLT \uh,\opLT \vh) = (F,\opLT \vh), \quad\forall \vh \in V_h
% \end{align}
% In the Galerkin Least Square method, we combine the standard Galerkin and the Least Square method. That is, we can formulate the problem as follows, find $\uh\in V_h$ such that:
\begin{align} 
    (\opLT \uh, \vh) + \glspar(\opLT \uh,\opLT \vh)_h &= (F,\vh) + \glspar(F,\opLT \vh)_h, \quad\forall \vh \in V_h,\\
    \implies (\opLT \uh, \vh + \glspar\opLT \vh)_h &= (F,\vh + \glspar\opLT \vh)_h, \quad\forall \vh \in V_h,
    \label{eq:gls-abstract}
\end{align}
where $\glspar$ is a positive parameter to be chosen later.
Thus, given $ \adv \in \spaceVdiv $ and $ F \in L^2(\stDom) $, the discrete variational problem with Galerkin--least-square stabilization reads as: find $\uh \in V_h$ such that
\begin{align}\label{def:discrete-variational-form}
    \bformh(\uh,\vh) = \lformh(\vh) \quad\forall \vh \in V_h,
\end{align}
where the discrete bilinear form $\bformh(\uh,\vh)$ and linear form $\lformh(\vh)$ are as follows:
\begin{align}\label{def:discrete-bilinear-form}
\begin{split}
    \bformh(\uh,\vh) &= (\uht,\vh) + (\adiv\uh, \vh) + (\visco\grad\uh,\grad\vh)\\
    &\quad +\innerh{\glspar [\uht + \adiv \uh- \visco\laplacian \uh]}{[\vht + \adiv \vh- \visco\laplacian\vh]},
\end{split}\\
\label{def:discrete-linear-form}
\lformh(\vh) &= \inner{F}{\vh} + \innerh{F}{[\vht + \adiv \vh- \visco\laplacian\vh]}. % (F,(\vh+\glspar\vht+\glspar\adv\cdot\grad\vh-\glspar\grad\cdot(\visco\grad\vh))).
\end{align}

\begin{remark}
	The Galerkin--Least-square formulation \eqref{eq:gls-abstract} is consistent, i.e., the exact solution $u$ satisfies \eqref{eq:gls-abstract}. We can rewrite \eqref{eq:gls-abstract} as
	\begin{align}
	\innerh{\opLT \uh - F}{\vh + \glspar\opLT \vh} &= 0.
	\end{align}
	Now, if we substitute $ \uh = u $ in the left hand side of the above equation, we have
	\begin{align}\label{eq:gls-abstract-for-exact-solution}
	\innerh{\opLT u - F}{\vh + \glspar\opLT \vh} &= 0 \ \ \forall \vh \in \spaceVh
	\end{align}
	because $ \opLT u - F = 0 $ pointwise (see \eqref{pde-mod:linear-advection-diffusion-equation}). It follows that 
	\begin{align}\label{eq:exact-solution-discrete-form}
	\bformh(u,\vh) = \lformh(\vh) \quad\forall \vh \in \spaceVh
	\end{align}
\end{remark}
\begin{remark}\label{remark:galerkin-orthogonality}
	Subtracting \eqref{eq:exact-solution-discrete-form} from  \eqref{def:discrete-variational-form}, we get the so-called Galerkin orthogonality:
	\begin{align*}
	\bformh(\uh-u,\vh) = 0 \quad\forall \vh \in \spaceVh.
	\end{align*}
\end{remark}
\begin{remark} \label{remark:stabilization}
	The stabilization parameter $ \glspar $ for the space-time problem \eqref{def:discrete-variational-form} is adapted from existing estimates of such parameters \cite{codina2000stabilized}, and expressed as
	\begin{align}
	\glspar_K = \left[ \frac{c_1}{\he^2} \ellipticAmat_0 + \frac{c_2}{\he} \ellipticBvec_0 \right]^{-1},
	\end{align}
	where
	\begin{align}
	\ellipticAmat_0 = \sqrt{\ellipticA_{ij}\ellipticA_{ij}},\ \ \ellipticBvec_0 = \sqrt{\ellipticB_i \ellipticB_i},\ \text{and}\ c_1,c_2 >0 \ \text{are some constants}.
	\end{align}
	$ \ellipticAmat $ and $ \ellipticBvec $ are defined in \eqref{expr:ellipticity-matrix-original}. An alternative definition of $ \glspar $ can be found in \cite{shakib1991new}.
	
	If $ \ellipticAmat $ and $ \ellipticBvec $ are constants, and $ \frac{\ellipticAmat_0}{\ellipticBvec_0} \ll (\nicefrac{c_2}{c_1})\he $, i.e., when advection dominates, then $ \glspar \propto \he$. On the other hand, $ \glspar \propto \he^2 $ when diffusion dominates (i.e., $ \frac{\ellipticAmat_0}{\ellipticBvec_0} \gg (\nicefrac{c_2}{c_1})\he $).
\end{remark}
%Clearly, $ [\bform(v,w); l(w)] $ (equations \eqref{def:discrete-bilinear-form} and \eqref{def:discrete-linear-form}) are different from $ [\bformh(v,w); l^h(w)] $ (equations \eqref{def:continuous-bilinear-form} and \eqref{def:continuous-linear-form}).

%When we use linear basis functions, the inner products containing the higher order derivative terms do not contribute.
%In the following formulation we assume the approximate solution in a linear polynomial space and thus all the terms with degree higher than or equal to 2 vanish. Thus we work with a truncated version of the discrete bilinear form:
%\begin{align}\label{def:discrete-bilinear-form-truncated}
%\begin{split}
%    \bformh(\uh,\vh) &= (\uht,\vh) + (\adv\cdot\grad\uh, \vh) + (\visco\grad\uh,\grad\vh) \\
%    &\quad +\glspar(\uht,\vht) + \glspar(\uht,\adv\cdot\grad\vh)+\glspar(\grad\uht,\visco\grad\vh)\\
%    &\quad +\glspar(\adv\cdot\grad\uh,\vht)+\glspar(\adv\cdot\grad\uh,\adv\cdot\grad\vh)
%    +\glspar(\visco\grad\uh,\grad\vht)
%\end{split}
%\end{align}
%\begin{align}\label{def:discrete-linear-form-truncated}
%    l^h(\vh) = (F,(\vh+\glspar\vht+\glspar\adv\cdot\grad\vh))
%\end{align}

\subsection{Analysis of the stabilized formulations}
We now turn to the analysis of stability and convergence of the method discussed in the previous section. We will prove the stability and the convergence estimates in the following discrete norm:
\begin{align}
\normVh{\uh} := \left[\norm{\uh}_{\bft}^2 + \norm{\grad\uh}^2 + \normh{\glspar^{\halfnice}[\uht + \adiv\uh - \visco\laplacian\uh]}^2\right]^{\halfnice}
\end{align}
We also define an auxiliary norm as follows:
\begin{align}
\normVhstar{\uh}^2 = \left(\norm{\uht}^2 + \normVh{\uh}^2\right)^{\halfnice}.
\end{align}
We will use both these norms in the sequel to prove the stability and boundedness of the discrete bilinear form \eqref{def:discrete-bilinear-form}.

\begin{lemma}[Boundedness]\label{lemma:boundedness}
	For $ \adv \in \spaceVdiv $ and $ \uh,\ \vh \in \spaceVh $, the bilinear form \eqref{def:discrete-bilinear-form} is uniformly bounded on $V_h\times V_h$, i.e.,
	\begin{align}
		|\bformh(\uh,\vh)|\leq\mu_b \normVhstar{\uh} \normVh{\vh}.
	\end{align}
\end{lemma}
\begin{proof}
	See \ref{sec:proof-boundedness}.
\end{proof}

\begin{lemma}[Coercivity]\label{lemma:coercivity-stability}
If $ \adv \in \spaceVdiv $ and $ \uh \in \spaceVh $, then
\begin{align*}
    \bformh(\uh,\uh) \geq \mu_c\normVh{\uh}^2, \textrm{ for some }\mu_c > 0.
\end{align*}
\end{lemma}
\begin{proof}
	See \ref{sec:proof-coercivity}.
\end{proof}

\lemref{lemma:coercivity-stability} imply that \eqref{def:discrete-variational-form} has a unique solution.

\begin{corollary}
	Given $ \adv \in \spaceVdiv $, there exists a unique solution of \eqref{def:discrete-variational-form}.
\end{corollary}
\begin{proof}
	From \eqref{def:discrete-linear-form}, we have
	\begin{align*}
	|\lformh(\vh)| &\leq |\inner{F}{\vh}| + |\innerh{F}{[\vht + \adiv \vh- \visco\laplacian\vh]}| \\
	&\leq \norm{F}\norm{\vh} + \normh{\glspar^{\halfnice} F} \normh{\glspar^{\halfnice} \opLT \uh} \\
	&\leq \left[ \norm{F}^2 + \normh{\glspar^{\halfnice} F}^2 \right]^{\halfnice} \left[ \norm{\vh}^2 + \normh{\glspar^{\halfnice} \opLT \uh}^2 \right]^{\halfnice}.
	\end{align*}
	Defining
	\begin{align*}
	 \normVhstar{F} = \left[ \norm{F}^2 + \normh{\glspar^{\halfnice} F}^2 \right]^{\halfnice},
	\end{align*}
	and using $ \norm{\vh} \leq \norm{\grad \vh} $, we have
	\begin{align*}
	|\lformh(\vh)| &\leq \normVhstar{F} \normVh{\vh}.
	\end{align*}
	This proves that the linear form $ \lformh $ is continuous. Since by \lemref{lemma:boundedness} and \lemref{lemma:coercivity-stability}, we also have that the discrete bilinear form $ \bformh $ is both bounded and coercive, therefore by the Lax-Milgram Lemma \cite{larson2013finite, jt1976introduction}, \eqref{def:discrete-variational-form} has a unique solution in $ \spaceVh $.
%	Assume $ {\uh}_1 $ and $ {\uh}_2 $ are two solutions of \eqref{def:discrete-variational-form}. Then,
%	\begin{align*}
%	\bformh({\uh}_1,\vh) &= \lformh(\vh) \quad\forall \vh \in V_h, \\
%	\bformh({\uh}_2,\vh) &= \lformh(\vh) \quad\forall \vh \in V_h.
%	\end{align*}
%	Subtracting,
%	\begin{align}
%	\bformh({\uh}_1-{\uh}_2, \vh) = 0 \quad\forall \vh \in V_h.
%	\end{align}
%	Choosing $ \vh = {\uh}_1 - {\uh}_2 $, and \lemref{lemma:coercivity-stability}, we have
%	\begin{align*}
%	0 = \bformh({\uh}_1-{\uh}_2,{\uh}_1-{\uh}_2) \geq \mu_c \normVh{{\uh}_1-{\uh}_2}^2,
%	\end{align*}
%	which implies that $ {\uh}_1 = {\uh}_2 $.
\end{proof}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% To derive the boundedness of the operator, we need some auxiliary results:
% The following two inverse inequalities hold:
% \begin{align}\label{ineq:inv0}
%     \left\|v\right\|_{L^2(\partial K)}\leq C_{inv,0}h^{-1/2}_{K}\left\|v\right\|_{L^2(K)}
% \end{align}
% and
% \begin{align}\label{ineq:inv1}
%     \left\|\nabla_{ST}v\right\|_{L^2(K)}\leq C_{inv,1}h^{-1}_{K}\left\|v\right\|_{L^2(K)}
% \end{align}
% where $K$ is an arbitrary element in the mesh $\mathcal{K_h}$ and $\nabla_{ST}$ is the gradient operator including all first derivatives, i.e., $\nabla_{ST} = (\partial_x,\partial_y,\partial_z,\partial_t)$

% Thus, from inequality \ref{ineq:inv1}, we can further write:
% \begin{align}
%     \left\|\partial_t v\right\|_{L^2(K)}\leq C_{inv,1}h^{-1}_{K}\left\|v\right\|_{L^2(K)}
% \end{align}
% We can also look at $\nabla_{ST}$ as $\nabla_{ST} = (\nabla_s,\partial_t)$, where $\nabla_s$ is the gradient operator on just the spatial variables (we have been using the notation $\nabla$ in place of $\nabla_s$ till now and will continue use the same way hereafter; we use the subscript 's' for emphasis here). And from this consideration, we can further write,
% \begin{align}
%     \left\|\partial_t \partial_{x_i}v\right\|_{L^2(K)}\leq C_{inv,1}h^{-1}_{K}\left\|\partial_{x_i}v\right\|_{L^2(K)}
% \end{align}

% Now, in expression \ref{exp:gls-bilinear-form}, the first, second and the third terms can be easily bounded in the same way as in section \ref{subsubsec:boundedness-bilinear-unstab}, i.e., by use of the Cauchy-Schwarz inequality. The fourth term can be bounded as follows:

% \begin{align}
%     \delta \Big(\nabla(u_t),\visco\nabla v\Big) 
%     & \leq  \delta\visco \left\| \nabla(u_t) \right\|_{L^2(\stDom_{ST})}\left\| \nabla(v) \right\|_{L^2(\stDom_{ST})}\\
%     & \leq  \delta\visco C_{inv,1}h^{-1} \left\| u \right\|_{H^1(\stDom_{ST})}\left\| v \right\|_{H^1(\stDom_{ST})}
% \end{align}
% And the last term can be bounded similarly. So, finally,
% \begin{align}
%     |A(u,v)| \leq C \left\| u \right\|_{H^1(\stDom_{ST})}\left\| v \right\|_{H^1(\stDom_{ST})}
% \end{align}

% This is easy enough, but using the $H^1$-norm makes error analysis complicated. Thus we will have to construct a norm that is closer to the bilinear form, so that error estimation becomes natural. This is done in \eqref{def:norm-v}. Therefore, we now have to show boundedness with respect to this norm. We do this taking each of the inner products appearing in \ref{exp:gls-bilinear-form}.

% \begin{enumerate}[I]
%     \item 
%     The first inner product
%     \begin{align*}
%         \Big(u_t,v\Big) & = \large\int_{\stDom_{ST}}u_tvdQ = -\large\int_{\stDom_{ST}}uv_tdQ + \large\int_{\Gamma_T}uvds\\
%         &\leq \left(\delta^{-1}\|u\|^2_{L^2(\stDom_{ST})}\right)^{\frac{1}{2}} \left(\delta\|\partial_t v\|^2_{L^2(\stDom_{ST})}\right)^{\frac{1}{2}}
%         +\Big(\|u\|^2_{L^2(\Gamma_T)}\Big)^{\frac{1}{2}}\Big(\|v\|^2_{L^2(\Gamma_T)}\Big)^{\frac{1}{2}}
%     \end{align*}
    
%     \item
%     The second inner product
%     \begin{align*}
%         \Big(\visco \nabla u, \nabla v\Big) 
%         \leq \Big(\visco \|\nabla_s u\|^2_{L^2(\stDom_{ST})}\Big)^{\frac{1}{2}}\Big(\visco \|\nabla_s v\|^2_{L^2(\stDom_{ST})}\Big)^{\frac{1}{2}}
%     \end{align*}
    
%     \item
%     The third inner product
%     \begin{align*}
%         \delta\Big(u_t,v_t\Big) \leq
%         \Big(\delta \|\partial_t u\|^2_{L^2(\stDom_{ST})}\Big)^{\frac{1}{2}}
%         \Big(\delta \|\partial_t v\|^2_{L^2(\stDom_{ST})}\Big)^{\frac{1}{2}}
%     \end{align*}
    
%     \item 
%     % We look at the last two terms together
%     % \begin{align*}
%     %     \delta \Big(\nabla_s(u_t),\visco\nabla_s v\Big)
%     %     +\delta \Big(\visco\nabla_s u,\nabla_s(v_t)\Big)
%     %     & = 
%     %     \delta \Big(\nabla_s(u_t),\visco\nabla_s v\Big)
%     %     +\delta \large\int^T_0 \large\int_{\stDom_S} (\visco \nabla_s u)\cdot \frac{\partial}{\partial t}(\nabla_s v) d\stDom_S dt\\
%     %     & = 
%     %     \delta \Big(\nabla_s(u_t),\visco\nabla_s v\Big)
%     %     -\delta \large\int^T_0 \large\int_{\stDom_S} (\visco \frac{\partial}{\partial t}\nabla_s u)\cdot (\nabla_s v) d\stDom_S dt\\
%     %     & + \delta \Bigg[\large\int_{\stDom_s \times \{T\}} \visco \nabla_s u_T \cdot \nabla_s v_T dS 
%     %     -\large\int_{\stDom_s \times \{0\}} \visco \nabla_s u_0 \cdot \nabla_s v_0 dS
%     %     \Bigg]\\
%     %     & = \delta \Big(\nabla_s(u_t),\visco\nabla_s v\Big)
%     %     -\delta \Big(\nabla_s(u_t),\visco\nabla_s v\Big) + \delta \Bigg[\large\int_{\stDom_s \times \{T\}} \visco \nabla_s u_T \cdot \nabla_s v_T dS\Bigg]\\
%     %      & = \delta \Bigg[\large\int_{\stDom_s \times \{T\}} \visco \nabla_s u_T \cdot \nabla_s v_T dS\Bigg]\\
%     %      & \leq \delta \Big(\visco \|\nabla_su_T\|^2_{L^2(\Gamma_T)}\Big)^{\frac{1}{2}}\Big(\visco \|\nabla_sv_T\|^2_{L^2(\Gamma_T)}\Big)^{\frac{1}{2}}
%     %      & \leq 
%     % \end{align*}
%     The fourth inner product
%     \begin{align*}
%         \delta \Big(\nabla_s(\partial_t u), \visco \nabla_s v\Big)
%         & \leq\Big(\visco \|\nabla_s u\|^2_{L^2(\stDom_{ST})}\Big)^{\frac{1}{2}}\Big(\delta^2\visco \|\partial_t \nabla_s v\|^2_{L^2(\stDom_{ST})}\Big)^{\frac{1}{2}}\\
%         & \leq\Big(\visco \|\nabla_s u\|^2_{L^2(\stDom_{ST})}\Big)^{\frac{1}{2}}
%         \Big(\delta^2\visco \sum^d_{i=1}\sum_{K\in\mathcal{K_h}}\|\partial_t (\partial_{x_i}v)\|^2_{L^2(\stDom_{ST})}\Big)^{\frac{1}{2}}\\
%         & \leq\Big(\visco \|\nabla_s u\|^2_{L^2(\stDom_{ST})}\Big)^{\frac{1}{2}}
%         \Big(\delta^2\visco C_{inv,1}^2 \sum^d_{i=1}\sum_{K\in\mathcal{K_h}}h_K^{-2}\|\partial_{x_i}v\|^2_{L^2(\stDom_{ST})}\Big)^{\frac{1}{2}}\\
%         & \leq\Big(\visco \|\nabla_s u\|^2_{L^2(\stDom_{ST})}\Big)^{\frac{1}{2}}
%         \Big(\delta^2\visco C_h^2 C_{inv,1}^2h^{-2} \|\nabla_sv\|^2_{L^2(\stDom_{ST})}\Big)^{\frac{1}{2}}\\
%     \end{align*}
    
%     \item
%     The fifth inner product is similar to the fourth one, so,
%     \begin{align*}
%         \delta \Big(\nabla_s u, \visco \nabla_s(\partial_t v)\Big)
%         & \leq \Big(\delta^2\visco C_h^2 C_{inv,1}^2h^{-2} \|\nabla_su\|^2_{L^2(\stDom_{ST})}\Big)^{\frac{1}{2}}
%         \Big(\visco \|\nabla_s v\|^2_{L^2(\stDom_{ST})}\Big)^{\frac{1}{2}}
%     \end{align*}
% \end{enumerate}
% Now making use of the Cauchy-Schwarz inequality, we get,
% \begin{align*}
%     |A(u,v)| & \leq
%     \Bigg[\delta^{-1}\|u\|^2_{L^2(\stDom_{ST})} + \|u\|^2_{L^2(\Gamma_T)} + \visco \|\nabla_s u\|^2_{L^2(\stDom_{ST})} + \delta \|\partial_t u\|^2_{L^2(\stDom_{ST})} 
%     \\& \qquad + \visco \|\nabla_s u\|^2_{L^2(\stDom_{ST})} + \delta^2\visco C_h^2 C_{inv,1}^2h^{-2} \|\nabla_su\|^2_{L^2(\stDom_{ST})}\Bigg]^{\frac{1}{2}}
%     \\& \qquad  \times \Bigg[\delta\|\partial_t v\|^2_{L^2(\stDom_{ST})} + \|v\|^2_{L^2(\Gamma_T)}
%     + \visco \|\nabla_s v\|^2_{L^2(\stDom_{ST})}\\
%     &  \qquad + \delta^2\visco C_h^2 C_{inv,1}^2h^{-2} \|\nabla_sv\|^2_{L^2(\stDom_{ST})}
%     +\visco \|\nabla_s v\|^2_{L^2(\stDom_{ST})}
%     \Bigg]^{\frac{1}{2}}
%     \\
%     \implies |A(u,v)| & \leq
%     \Bigg[\delta^{-1}\|u\|^2_{L^2(\stDom_{ST})} + \|u\|^2_{L^2(\Gamma_T)} + \delta \|\partial_t u\|^2_{L^2(\stDom_{ST})} +
%      \left(2 + \delta^2 C_h^2 C_{inv,1}^2h^{-2}\right)\visco \|\nabla_su\|^2_{L^2(\stDom_{ST})}\Bigg]^{\frac{1}{2}}
%     \\& \qquad \times \Bigg[\|v\|^2_{L^2(\Gamma_T)} + \delta\|\partial_t v\|^2_{L^2(\stDom_{ST})} 
%     +\ \left(2 + \delta^2 C_h^2 C_{inv,1}^2h^{-2}\right)\visco \|\nabla_s v\|^2_{L^2(\stDom_{ST})}
%     \Bigg]^{\frac{1}{2}}
%     \\
%     \implies |A(u,v)| & \leq
%     \mu_b \|u\|_{\spDom}\|v\|_{V}
% \end{align*}
% where $\|v\|_{V}$ is defined in \eqref{def:norm-v} and $\|u\|_{\spDom}$ is defined as follows:
% \begin{align}
%     \|u\|_{\spDom} = \left[\|v\|_{V} + \delta^{-1}\|u\|^2_{L^2(\stDom_{ST})}\right]^{\frac{1}{2}}
% \end{align}

% Finally $\mu_b$ can be chosen as $\mu_b = \big[2 \textrm{ max}\{1,\frac{\delta^2 C_h^2 C_{inv,1}^2h^{-2}}{2}\}\big]^{\frac{1}{2}}$
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsubsection{Boundedness of the linear functional}
% From the definition of the linear form $L(v)$ in expression \ref{exp:gls-linear-form},
% \begin{align*}
%     |L(v)| &= |(f,v+\delta v_t)|\\
%     &\leq \|f\|_{L^2(\stDom_{ST})} \Big( \|v\|_{L^2(\stDom_{ST})} + \|v_t\|_{L^2(\stDom_{ST})}\Big)\\
%     &\leq \|f\|\|v\|_{H^1}
% \end{align*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{A priori error analysis}
In this section, we derive \textit{a priori} error estimates for the GLS stabilized space-time advection diffusion equation. In \eqref{pde-mod:linear-advection-diffusion}, we assume that the exact solution $ u \in \spaceV \cap H^m(\stDom) $ (using regularity estimates from Section 6.3 in \cite{evans2022partial}), and consequently the forcing  $ F \in L^2(\stDom) \cap H^{m-2}(\stDom) $. To establish the error estimates, we consider an interpolant $ \interp{u} : \spaceV \cap H^m(\stDom) \rightarrow \spaceVh $. Then we have the following estimates for the distance between $ u $ and $ \interp{u} $.
%\begin{lemma}[Regularity]
%If $\adv: \stDom \rightarrow \mathbb{R}^n$ and $\visco: \stDom \rightarrow \mathbb{R}$ in \ref{pde:linear-advection-diffusion} are smooth and the right hand side $F: \stDom \rightarrow \mathbb{R} \in L^2(\stDom)$ then $v\in H^2_{loc}(\stDom)$.
%\end{lemma}
%\begin{proof}
%	The proof follows from Theorem 2 in Section 6.3 (Regularity) of \cite{evans2022partial}.
%\end{proof}
\begin{lemma}[Approximation estimate in a Sobolev space]\label{estimate:sobolev-approximation}
Let $\interpolant$ be the interpolation operator from $ \spaceV \cap H^m(\stDom) $ to $\spaceVh$, with order of interpolation $k \in \mathbb{N}$. Also, let $ l \in \mathbb{N} $. If $k, l, m $ satisfy $0\leq l \leq (k+1) \leq m $, then
\begin{align*}
    \normH[l]{v-\interp{v}}{\stDom}\leq \approxConstant h^{(k+1-l)}\seminormH[k+1]{v}{\stDom},
\end{align*}
where the constant $\approxConstant$ only depends on $k,l,m$ and is independent of $h$ and $v$.
\end{lemma}
\begin{proof}
The proof follows from the technique outlined in Section 4.4 of \cite{brenner2007mathematical} and Section 6.7 of \cite{jt1976introduction}.
\end{proof}
\begin{remark}
The following estimates are direct consequences of \lemref{estimate:sobolev-approximation} on any element $ K \in \mesh $ (assuming $m=k+1$).
\begin{subequations}\label{estimate:sobolev-interp}
	\begin{align}
	\normL{v-\interp{v}}{K} &\leq {\approxConstant}_0 \he^{k+1}\seminormH[k+1]{v}{K},
	\label{estimate:sobolev-interp-L2}\\
	\normL{\grad (v-\interp{v})}{K} &\leq {\approxConstant}_1 \he^{k}\seminormH[k+1]{v}{K},
	\label{estimate:sobolev-interp-grad-L2}\\
	\normL{\partial_t(v-\interp{v})}{K} &\leq {\approxConstant}_1 \he^{k}\seminormH[k+1]{v}{K}.
	\label{estimate:sobolev-interp-time-der-L2} \\
	\normL{\laplacian (v-\interp{v})}{K} &\leq {\approxConstant}_2 \he^{k-1}\seminormH[k+1]{v}{K},
	\label{estimate:sobolev-interp-laplacian-L2}
	\end{align}
\end{subequations}
\begin{corollary} \label{lemma:interp-boundary-estimate}
	For the final time boundary $ \bft $, we similarly have
	\begin{align}
	\normL{v-\interp{v}}{\partial K} 
	&\leq C_{a\Gamma} \he^{k+\frac{1}{2}}|v|_{H^{k+1}(K)}.
	\label{estimate:sobolev-interp-boundary-L2}
	\end{align}
\end{corollary}
\begin{proof}
	See \ref{sec:proof-interp-boundary}.
\end{proof}
\end{remark}
% \begin{lemma}\label{estimate:scaled-trace-inequality}
% Assume each element $K\in\mesh$ has Lipschitz continuous boundary $\partial K$ and has diameter $h_K$. Then the following scaled trace inequality
% \begin{align*}
%     \normL{v}{\partial K} \leq \traceConstant \left( h_K^{-1}\normL{v}{K}^2 + h_K\normH{v}{K}^2 \right)^{\frac{1}{2}}
% \end{align*}
% holds for all $v\in H^1(K)$ where $\traceConstant>0$ does not depend on $v$.
% \end{lemma}
\begin{lemma}\label{lemma:interp-estimate-in-Vh}
Let $ u \in \spaceV \cap H^m(\stDom) $, and suppose $ \interpolant: \spaceV \cap H^m(\stDom) \rightarrow \spaceVh  $ is the projection of $u$ from $\spaceV$ to $\spaceVh$. Assume that $ \interpolant $ has the degree of interpolation $ k \in \mathbb{N} $ such that $ k+1 < m $. If $ m \geq 2 $, then the following estimate holds,
%Let $k \in \mathbb{N}$ be the degree of interpolation of $ \interp{u} $ such that $ k+1 \leq m $ be a fixed integer and $l, m$ integers such that $0 \leq m \leq k+1$. Let $\interpolant$ be the interpolation operator from $H^m(\stDom) \cap \spaceV$ to $\spaceVh$. If $v \in \spaceV \cap H^m(\stDom), m>2$ and $\interp{v}$ is the projection of $v$ from $\spaceV$ to $\spaceVh$, then the following estimate holds,
\begin{align*}
    \normVh{\interp{u}-u} \leq C h^{k}\seminormH[k+1]{u}{\stDom}
\end{align*}
for some $C>0$.
\end{lemma}
\begin{proof}
	See \ref{proof:interp-estimate-vh}.
\end{proof}

% \begin{corollary}
% Since we also have $\normL{v-\interp{v}}{\stDom} \leq \approxConstant^2h^{k+1}\seminormH[k+1]{v}{\stDom}$, therefore it directly follows that
% \begin{align*}
%     \normVstar{v-\interp{v}} \leq C h^{k}\seminormH[k+1]{v}{\stDom}
% \end{align*}
% \end{corollary}
\begin{theorem}\label{theorem:a-priori-estimate}
If $u \in V\cap H^m(\stDom)$ is the exact solution to \eqref{pde-mod:linear-advection-diffusion} and $\uh\in V_h$ is the exact solution to the finite element problem \eqref{def:discrete-variational-form}. If the degree of the basis functions in $ \spaceVh $ is $ k $, then the discretization error estimate satisfies,
\begin{align*}
    \normVh{\uh-u}\leq C h^{k}\normH[k+1]{u}{\stDom}
\end{align*}
for some $C>0$.
\end{theorem}
\begin{proof}
	See \ref{sec:proof-a-priori}.
\end{proof}


% There are total five inner products in $A(u,v)$. Treating them one by one sequentially:
% \begin{enumerate}[I]
%     \item
%     \begin{align}
%         \Big(\frac{\partial (u-\pi u)}{\partial t},u_h-\pi u\Big)
%         & = \left\|\frac{\partial (u-\pi u)}{\partial t}\right\|_{L^2(\stDom_{ST})}  \left\|u_h-\pi u\right\|_{L^2(\stDom_{ST})}\\
%         & \leq C_{inv,1}h^{-1}\left\|(u-\pi u)\right\|_{L^2(\stDom_{ST})}  \left\|u_h-\pi u\right\|_{L^2(\stDom_{ST})}\\
%         & \leq C_{inv,1}h^{-1}h^2\left\|u\right\|_{H^2(\stDom_{ST})}  \left\|u_h-\pi u\right\|_{L^2(\stDom_{ST})}\\
%         & \leq C_{inv,1}h\left\|u\right\|_{H^2(\stDom_{ST})}  \left\|u_h-\pi u\right\|_{L^2(\stDom_{ST})}
%     \end{align}
% \end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{A posteriori error analysis}
In addition to solving \eqref{def:discrete-bilinear-form} in space-time, we would also like to perform adaptive refinement of the space-time mesh $ \mesh $. To this end, we use the following residual-based \textit{a posteriori} error indicator for each element $ K $ in $ \mesh $:
\begin{align*}
\etaElm = \left[ h_K^2\|r\|_K^2 + \frac{1}{2}\Xsum_{E\in\mathcal{E}_K}h_E\|j\|_E^2 \right]^{\halfnice},
\end{align*}
where $ \he $ is the size of the element $ K $, and $ \mathcal{E}_K $ is the set of all the boundaries of element $ K $. The PDE-residual $ r $ and the jump-residual $ j $ are defined as
\begin{subequations}
	\begin{align}
	r|_K &= F - \opLT \uh \ \ \text{on every} \ K \in \mesh, \\
	j|_E &= \begin{cases}
	0\ \ \text{if} \ E \in \bit \cup \bsp,\\
	-\jump(\ddiv{\normalvec_E}\uh),\ \ \text{otherwise}.
	\end{cases}
	\end{align}
\end{subequations}
The jump operator $ \jump $ acting on a function $ \vh $ is defined as
\begin{align}
\jump_E \vh(\xvec) = \lim_{t\rightarrow 0^+} \vh(\xvec - t\normalvec_E) - \lim_{t\rightarrow 0^+} \vh(\xvec + t\normalvec_E) ,\ E \in \edgeset,
\end{align}
$\edgeset$ being the set of all the edges of all the elements in the mesh $\mesh$. The cumulative error indicator $ \eta $ can be defined as
\begin{align}
\etaFull := \left(\elmsum \etaElm^2 \right)^{\halfnice}.
\end{align}
The next theorem shows that the cumulative error indicator bounds the true error.
\begin{theorem}\label{theorem:a-posteriori-estimate}
If $ u $ is the solution of \eqref{pde-mod:linear-advection-diffusion} and $ \uh \in \spaceVh $ is the solution of \eqref{def:discrete-variational-form}, then 
	\begin{align}
	\normVhstar{u-\uh} 
	&\leq C\etaFull.
	\end{align}
\end{theorem}
\begin{proof}
	See \ref{sec:proof-a-posteriori}.
\end{proof}
% \end{document}

==> sections/3_implementation_details.tex <==
% \documentclass[../main.tex]{subfiles}
% \begin{document}
%################################# SECTION ##########################################
%################################# SECTION ##########################################
%################################# SECTION ##########################################
%################################# SECTION ##########################################

\section{Implementation Details}\label{sec:implementation-details}

The inclusion of time as an additional dimension results in a higher dimensional domain and consequently the meshes too. Thus the mesh for a 1-D, 2-D and 3-D domains result in 2-D, 3-D and 4-D meshes respectively. This allows for using the same polynomial degree in the time direction as being used in the space directions.

The present methodology was implemented through our in-house scalable parallel finite-element analysis software written in C++. It is optimized for distributed memory computing. This program in turn uses PETSc for the parallel matrix and vector data structures as well as the linear algebra routines. The spacetime formulation results in a system of equation that is not symmetric. Thus Krylov methods such as conjugate gradients and biconjugate gradient methods do not provide good parallel performance. GMRES works very well, especially with preconditioners such as block Jacobi, generalized ASM as well as SOR type and algebraic multigrid type preconditioners. Multigrid preconditioners provide marginal advantage in solve time but has a higher memory requirement.

% \end{document}

==> sections/4_num_examples.tex <==
% \documentclass[../main.tex]{subfiles}
% \begin{document}
%################################# SECTION ##########################################
%################################# SECTION ##########################################
%################################# SECTION ##########################################
%################################# SECTION ##########################################
\section{Numerical Examples}\label{sec:numerical-examples}
In this section we look at three specific examples modeled by \eqref{pde:linear-advection-diffusion}. These special cases are: \textit{(i)} the heat equation ($\adv = \underline{0}\text{ , }\visco \neq 0$), \textit{(ii)} the advection-diffusion equation (both $\adv \neq \underline{0} \text{ , }\visco \neq 0$) and \textit{(iii)} the transport equation ($\adv \neq \underline{0} \text{ , } \visco=0$, which is a hyperbolic equation). 

In the first two cases, we perform a convergence study with a known smooth analytical solution and confirm the results of a priori and a posteriori errors obtained in \secref{sec:math-formulation}. Then we discuss the nature of the uniform mesh solutions for the second and third cases and present comparisons with a sequential time-marching solution. Finally, we present results on the space-time adaptive solutions for all three cases.
In all examples, we take the space-time domain to be $\stDom = [0,1]^3 $.
  
\subsection{Convergence study}\label{subsec:conv-study}
% To study the convergence of the solution of both the heat equation and the advection-diffusion equation, we make use of known analytical solutions.
\input{sections/6_05a_case_1_convergence.tex}

\subsubsection{The heat equation}\label{subsubsec:convergence-heat-eq}
The linear heat equation is given by
\begin{align}
    \begin{cases}
        u_t - \grad \cdot(\visco\grad u) = f \qquad &\text{in } \stDom = (0,1)\times(0,1)\times(0,1]\\
        u = 0 & \text{on } \Gamma_s\\
        u = u_0(\mvec{x}) & \text{on } \Gamma_0\\
    \end{cases}
    \label{eq:numex-pde-heat-eq}
\end{align}
where $\visco = \visco (\underline{x},t)$ and the forcing $f = f(\underline{x},t)$.

If $f = 0$ in \eqref{eq:numex-pde-heat-eq}, then the analytical solution to \eqref{eq:numex-pde-heat-eq} is given by the single Fourier mode
\begin{align}
    u_{a} = e^{-2\pi^2\visco t}\sin{(\pi x)}\sin{(\pi y)}
\end{align}
with initial condition $u_0(x,y) = u_a(x,y,t=0) = \sin{(\pi x)}\sin{(\pi y)}$. 

This problem is then also solved through the formulation presented in \secref{sec:math-formulation} on different sizes of space-time mesh. 
\figref{fig:conv-study-case4-diff-expdecay} shows the plot of $\normL{u^h-u_a}{\stDom}$ along with $\etaFull$ against $h$ on a $\log-\log$ plot. The slope of this line in the $\log-\log$ plot is $2$, which is expected because linear basis functions were used in the FEM computations. Note that the space-time \textit{a posteriori} error indicator $\etaFull$ decreases as $\normL{u^h-u_a}{\stDom}$ decreases, thus proving the reliability of the indicator. We note that $ \etaFull $ need not decrease at the same rate as the $ L^2 $-error.

\subsubsection{The advection-diffusion equation}\label{subsubsec:convergence-adv-diff-eq}
The advection-diffusion equation is given by (once again $\stDom$ is a unit cube),
\begin{align}
    \begin{cases}
        u_t + \adv\cdot\grad u- \grad \cdot(\visco\grad u) = f \qquad &\text{in } \stDom = (0,1)\times(0,1)\times(0,1]\\
        u = 0 & \text{on } \Gamma_s\\
        u = u_0(\mvec{x}) & \text{on } \Gamma_0\\
    \end{cases}
    \label{eq:numex-adv-diff-pde}
\end{align}
We consider the analytical solution $u_a = e^{-t}\sin{(2\pi x)}\sin{(2\pi y})$ and analytically manufacture the forcing $f$ by substituting $u_a$ in \eqref{eq:numex-adv-diff-pde}. We solve this problem on a series of meshes with different levels of refinement and plot $\normL{u^h-u_a}{\stDom}$ and $\etaFull$ against $h$. This plot is shown in \figref{fig:conv-study-case1-ad-mms}. The space-time \textit{a posteriori} indicator follows a similar trend as the analytical error, thus proving its reliability.

% The other problem we consider for the heat equation, is where the heat source with Gaussian distribution is rotating in the $x-y$-plane. Note that this is rotation is not related to advection, because the initial condition is not being advected by a velocity field; rather the heat source itself is rotating which then causes the solution profile to rotate. In the next section, we will consider advective problems where the initial condition is advected by an existing velocity field in the absence of any force.

% The analytical solution for the rotating source diffusion problem is given by 
% \begin{equation}
%     u = e^{\frac{(x-x_0)^2 + (y-y_0)^2}{\sigma^2}}
% \end{equation}

% Figure ~\ref{fig:conv-study-case1-ad-mms} shows the convergence plot for an advection-diffusion problem where the forcing is manufactured with the solution:
% \begin{equation}
%     u = e^{-t}\sin(\pi x)\sin(\pi y)
% \end{equation}
% Once again, the \textit{a posteriori} error estimator decreases as the $L^2$-error decreases, thus proving the reliability of the indicator.
\input{sections/6_14_ad_case2_problem_def_schematic.tex}
\input{sections/6_15_ad_case2_comparison_sequential.tex}

\subsection{Uniform space-time mesh solutions and comparison to time-marching solutions}
\subsubsection{Advection-diffusion with smooth initial condition}\label{subsubsec:case2-smoothic}
We consider the two-dimensional, linear advection-diffusion equation \eqref{eq:numex-adv-diff-pde} where the advection field $\adv$ is purely rotational with unit angular velocity (see \figref{fig:initial-pulse-location}, \ref{fig:ad-case2-initial-condition}) and is given by 
\begin{align}
    \adv(\mvec{x}) = (-2\pi r_y, 2\pi r_x),
    \label{eq:numex-adv-field-rotating}
\end{align}
where $r_x$ and $r_y$ denote the distance of any point in the spatial domain from the center of the spatial domain $(\frac{1}{2},\frac{1}{2})$, i.e., $r_x=(x_1-0.5), r_y=(x_2-0.5)$. The speed of rotation is chosen in such a way that the pulse completes a full revolution at $t=1$.

The initial condition $u_0:U \rightarrow \mathbb{R}$ is a smooth function and is given by
% \begin{align}
%     u_0(\mvec{x}) = \begin{cases}
%     \frac{1}{4}(1+\cos\pi r_1)(1+\cos\pi r_2) & \text{if } (r_1^2 + r_2^2) \leq 1,\\
%     0 & \text{otherwise}
%     \end{cases}
%     \label{eq:numex-case2-initial-condition}
% \end{align}
\begin{align}
    u_0(\mvec{x}) = 
    e^{-\frac{(x-a)^2+(y-b)^2}{d^2}}.%\frac{1}{4}(1+\cos\pi r_1)(1+\cos\pi r_2) & \text{if } (r_1^2 + r_2^2) \leq 1
    \label{eq:numex-case2-initial-condition}
\end{align}
This is essentially a Gaussian pulse with its center at $(a,b)=\left(\frac{1}{3},\frac{1}{3}\right)$ and thickness at base $\approx 2d = 0.01$. The force $f$ on the right hand side is zero. The diffusivity value $\visco$ is fixed at $10^{-4}$. The initial pulse keeps rotating in the domain as time evolves. Since the advection field has unit angular velocity, thus theoretically the center of the pulse at $t=0$ and $t=1$ should coincide. Since the field is also diffusive, the height of the pulse reduces with time.

\figref{fig:case2-ad-uniref-7-threshold-view} shows contours of the solution $ u $ in space-time. For clarity, only some of the iso-surfaces close to the pulse are shown. The rotation of the pulse is evident from a helical structure of the figure. The total number of elements in this case is $128\times 128\times 128$ with each element being a trilinear Lagrange element.

To see how the space-time solution behaves in comparison to the time-marching methods, we choose the Crank-Nicolson scheme to solve the same problem. This is reasonable since Crank-Nicolson is the simplest second order implicit time-marching method. To compare the methods, we discretize $\stDom=(0,1)^2\times(0,1]$ with the same number of elements in each dimension. As an example, \figref{fig:case2-mesh-128-uniref-lev7-comparison} compares the solution contours obtained by the sequential method on a 2D $(128\times 128)$ mesh marching over $128$ time steps against a space-time solution in 3D using a $128^3$ mesh. The right column of plots in this figure shows a cross-section of the pulses at both $t=0$ and $t=1$ along the plane `AB', which passes through the center of initial pulse and is tangential to the local velocity vector (see \figref{fig:ad-case2-initial-condition}).

The Crank-Nicolson method is dispersive in nature and the solution exhibits a phase error; therefore the centers of the pulses between the two methods do not match. On the other hand, the space-time solution shows little dispersion and thus the peak centers align exactly. In regard to the undershoot around the pulse, the Crank-Nicolson solution shows a phase lag, whereas the space-time solution is visibly symmetric about the centre of the pulse. In both the solutions, however, the height of the peak at $t=1$ is roughly the same.

% In the same vein, Figure ~\ref{fig:case2-ad-ts-128} and \ref{fig:case2-ad-uniref-7} show the sequential and space-time results respectively when the discretization in each dimension is done through $128$ elements. In Figure ~\ref{plot:case2-ad-ts-128-plot-over-line} the pulse at the final time still exhibits a fair amount of dispersion, but the phase error is reduced. However, in Figure ~\ref{plot:case2-ad-uniref-7-plot-over-line}, the space-time solution show little dispersion and almost no phase error. And once again it can be noted that the pulse height at $t=1$ is roughly the same in both cases.
\subsubsection{Pure advection with a discontinuous initial condition}\label{subsubsec:case3-sharpic}

%\input{sections/6_16_ad_case3_problem_def_schematic.tex}
\input{sections/6_17_ad_case3_comparison_sequential.tex}

We solve \eqref{eq:numex-adv-diff-pde} with the same advection field mentioned in \eqref{eq:numex-adv-field-rotating} but this time with an initial condition that is not smooth in space. The initial data is given by,
\begin{align}
    u_0(\mvec{x}) = \begin{cases}
    1 & \text{if } (r_1^2 + r_2^2) \leq 1,\\
    0 & \text{otherwise},
    \end{cases}
    \label{eq:numex-case3-initial-condition}
\end{align}
where $\mvec{r} = (\mvec{x}-\mvec{x_0})/\sigma$. Here $\mvec{x_0} = \left(\frac{1}{3},\frac{1}{3}\right)$ is the initial position of the center of the circular pulse. The radius of this pulse is 1. Clearly, $u_0$ is discontinuous in space, (see \figref{fig:initial-pulse-location}, \ref{fig:ad-case3-initial-condition}).
The diffusivity value $\visco$ is set to $10^{-8}$ in this case. As earlier, the source term $f$ is zero. This choice of a negligible value of $\visco$ effectively renders this case as a purely advective one. The global Peclet number is given as $ Pe_g = \frac{\modulus{a}\cdot L}{\visco} \approx 4.4 \times 10^8 $. As in the previous case, we discretize this problem through space-time as well as sequential time marching schemes and compare the pulse at $t=0$ and $t=1$. \figref{fig:case3-mesh-128-uniref-lev7-comparison} shows this comparison for both sequential and space-time method for three sizes of discretizations: $ h=\oneOver{64}, \ \oneOver{128} $ and $  \oneOver{256} $. The corresponding mesh-Peclet numbers are $ Pe = \frac{\modulus{a}\cdot h}{2\visco} \approx 3.47\times 10^6, \ 1.74\times 10^6 $ and $ 8.68 \times 10^5 $ respectively. As in the previous example, the plots are line cuts of the pulse onto the plane `AB'.

%and \ref{fig:case3-ad-uniref-6} show the respective solutions when the discretization in each of the directions is done through $64$ elements. Similary Figures ~\ref{fig:case3-ad-ts-128} and \ref{fig:case3-ad-uniref-7} show the same when the discretization is $128$ in each direction.

It can be noticed rightaway that both sequential and space-time formulation have difficulty approximating the discontinuous pulse, which can be attributed to the use of continuous Galerkin approximation when attempting to model a solution that is discontinuous. The final time representation of the pulse gets smoothened out in both cases, albeit to a different degree. But once again, the Crank-Nicolson method exhibits higher dispersion and phase errors, whereas the spacetime solution has zero phase error and a smaller dispersion. Once again, as in the previous example, the undershoot in the Crank-Nicolson method only takes place in the upwind direction whereas there is typically no undershoot in the downwind direction. But the spacetime solution does not display any directional preference for the undershoot.

% \textbf{\emph{Temporal discretization}}: The final time in this simulation is $t = \pi$. Courant number is taken as 1. Once again we calculate the time step using the formula  $\Delta t = \frac{hC}{\|a\|}$. As mentioned above, $h = 1/30$. Now, $\|a\|$ is a depends on the coordinate values $(x_1,x_2)$ pointwise. So for calculating the time step, we use the maximum value of $\|\mathbf{a}\|$, i.e., $a$ at any of the corners of the square domain, those points where $|x| = \frac{1}{2}, |y| = \frac{1}{2}$. Thus, $\|a\| = \frac{1}{\sqrt{2}}$

% \textbf{\emph{Crank-Nicolson/Galerkin}}: This problem is solved using the continuous Galerkin method alongwith Crank-Nicolson scheme in time. The results are shown in figure \ref{fig:adv-rotating-cone-cn}.
% \subsubsection{Convergence}
% \subsubsection{The heat equation}
% \subsubsection{The advection diffusion equation}
%############################# Bicosine_Cone_2D ##################################
%############################# Bicosine_Cone_2D ##################################
%############################# Bicosine_Cone_2D ##################################
% \textbf{\emph{Advection diffusion, set $\nu = 10^{-5}$}}
% \textbf{\emph{Increasing the advection velocity:}} The velocity field is increased to $\mathbf{a}=(-2x_2, 2x_1)$, i.e., 2 times the previous field. The diffusivity is kept at $\nu=10^{-5}$.
% First let's look at the solution obtained with a reasonably fine mesh alongwith a moderately small value of the time-step. This is shown in figure \ref{fig:bicosine-seq-vel-times-2-fine-mesh-sol}.
% The velocity field is increased to $\mathbf{a}=(-5x_2, 5x_1)$. The diffusivity is kept at $\nu=10^{-5}$. The mesh is $72\times72$.

\subsection{Adaptive solutions}\label{subsec:adaptive-solutions}
% \subsection{Estimator behavior}\label{sec:estimator behavior}
%\input{sections/6_08_case5_diff_rotatingsource.tex}
The examples considered in the previous section have solutions that show a high degree of spatial as well as temporal localization. That is, at a given instance of time, the solution function has a significant change in value only at some small area of the whole domain and zero at all other points of the domain. Moreover, as time evolves, there is a limited region where the solution changes. A significant portion of the domain never experiences any change in the solution with the evolution of time. This can be observed in \figref{fig:case2-ad-uniref-7-threshold-view}, where the solution is zero in all of the white region. This kind of problems are therefore perfect candidates where space-time adaptive refinement strategy can be useful. To show the effectiveness of adaptive refinement in a space-time simulation, we consider the following three examples. 
% \begin{itemize}
%     \item A simple diffusion equation with a manufactured solution that exhibit high space-time localization.
%     \item The advection diffusion example problem defined by \ref{eq:numex-case2-case3-pde} and \ref{eq:numex-case2-initial-condition}.
%     \item The pure advectioin example problem defined by \ref{eq:numex-case2-case3-pde} and \ref{eq:numex-case3-initial-condition}.
% \end{itemize}

\subsubsection{The heat equation: estimator behavior in adaptive refinement}
\input{sections/6_09_case7_diff_gaussiansource.tex}
We begin with a simple heat diffusion problem to illustrate adaptive refinement in space-time. We go back to the heat \eqref{eq:numex-pde-heat-eq} with a forcing $f$ given by
\begin{align}
    f = - \left[ 2 + \visco \left(\frac{r_x^2+r_y^2}{d^4}\right) \left\{ 6+\frac{4}{d^4}(r_x^4 - r_x^2r_y^2 + r_y^4) \right\}\right]e^{-2t-\frac{r_x^2+r_y^2}{d^2}}.
    \label{eq:case7-gaussian-forcing}
\end{align}
The analytical solution is given by
\begin{align}
    u = e^{-2t-\frac{r_x^2+r_y^2}{d^2}}.
    \label{eq:case7-gaussian-u-analytical}
\end{align}
This problem describes a Gaussian pulse at the center of the spatial domain $U$ diffusing as time evolves.
In both \eqref{eq:case7-gaussian-forcing} and \eqref{eq:case7-gaussian-u-analytical}, $r_x = x-x_0$ and $r_y = y-y_0$, where $(x_0,y_0) = (\frac{1}{2},\frac{1}{2})$ is the center of the heat pulse, $d = 0.05$ is the ``thickness" of the pulse. The diffusivity $\visco = 0.01$ 

To solve this problem adaptively, we begin with a very coarse 3D octree mesh (representing 2D in space and 1D in time). After computing the FEM space-time solution on this coarse mesh, we use the \textit{a posteriori} error estimate presented in Theorem \ref{theorem:a-posteriori-estimate} to calculate the error indicator $\etaElm$ in each element ($K$ $\in$ $\mesh$). The elements, where the indicator $\etaElm$ is larger than a predetermined error tolerance, are refined. The refined mesh is then used to solve the same problem once again. This process is repeated for a few times till the error value in all the elements are smaller then the tolerance. \figref{fig:case5-diff-conv-compare-adref-uniref} shows comparisons of $\normL{u-u^h}{\stDom}$ and $ \etaFull $ for both uniform refinement and adaptive refinement. As expected, the error decreases much more rapidly when adaptive refinement is used.

A slice of the space-time mesh at the final refined state is shown in \figref{fig:case5-refined-mesh-slice-yt-plane}. The slice is a $y$-constant plane, therefore the levels of refinement in the time direction are visible in this image. The largest element size in this slice is $h_{max}=\frac{1}{2^3}=\frac{1}{8}$ whereas the smallest element size is $h_{min}=\frac{1}{2^7}=\frac{1}{128}$. The ratio of $h_{max}$ to $h_{min}$ is thus $16$.

\subsubsection{Advection-diffusion with smooth initial condition}\label{subsubsec:adref-case2-smoothic}
\input{sections/6_06_case2_ad_smoothic.tex}

\figref{fig:case2-adref-final-state-mesh-with-threshold} shows the pulse contour for the advection diffusion problem (solved earlier using a uniform space-time mesh) with a smooth initial condition, along with the adaptively refined space-time mesh. A 2D slice of the same mesh is shown in \figref{fig:case2-adref-final-state-mesh-slice-with-threshold}. \figref{fig:case2-adref-final-state-xy-slice} shows the mesh slice at $t=1$. As expected, the refinement is clustered around the smooth pulse. \figref{fig:case2-adref-final-state-yt-slice} on the other hand, shows a $y-t$ slice of the whole mesh. Once again, as seen from both these slices, the mesh size varies greatly between the finer and the coarser regions, which in this case, differs by a factor of $2^5$, i.e., the largest element has a size that is 32 times the size of the smallest element. Especially in relation to the mesh slice in \figref{fig:case2-adref-final-state-yt-slice}, it can be interpreted that different regions in the spatial domain are subjected to different ``time steps" to reach the same final time. This is a very different behavior compared to a sequential solution where every region in the spatial domain has to go through the same number of time steps to reach the final time. Moreover, in sequential methods, the size of this time-step is often constrained by the minimum size of the mesh. For example, in this problem, the error in the solution is higher near the peak of the pulse and is gradually less as distance from the peak increases in space-time. This indicates that to achieve a reasonable accuracy, the regions near the pulse need to be resolved at least by elements of size $\approx \frac{1}{2^8}$ in space. This then implies that when using implicit time-marching methods such as the Crank-Nicolson method, the time-step size also needs to be $\mathcal{O}(h)$. 

\figref{fig:case2-ad-adref-different-kappas} plots the cross-section of the pulse at $t=0$ and $t=1$ solved through both uniform-refinement and adaptive-refinement for four different values of $\visco$. For all of these four cases, the uniformly refined mesh is of size $128^3$, i.e., $\textsc{DOF} = 2146689$. The $\textsc{DOF}$ in the adaptive meshes vary from case to case. As an example, for the case of $\visco=10^{-8}$, the final refined state has $\textsc{DOF}=192507$.

Note that there is an appreciable decrease in the height of the pulse when $\visco = 10^{-4}$, but there is no such apparent loss when $\visco=10^{-6}$ or $\visco=10^{-8}$ which is correctly captured by the adaptive solutions. But the uniform $128^{3}$ mesh is unable to capture this; indicating that a further finer mesh is required. This shows that when $\visco$ is very low, it is very difficult to resolve the peak without resorting to extremely small mesh sizes. A final observation is that $\visco < 10^{-6}$ can be used to model a ``pure advection" case when considering $t\in[0,1]$ for this problem. Thus, this value of $\visco$ is used to model a ``purely advective" transport problem in the next example. 

\subsubsection{The advection-diffusion with sharp initial condition}\label{subsubsec:adref-case3-sharpic}
\input{sections/6_07_case3_ad_sharpic.tex}

Finally we  take a quick glance at the adaptive solution of the pure advection problem with a discontinuous initial data. This is the same problem discussed in \secref{subsubsec:case3-sharpic}. \figref{fig:case3-adref-final-state-contour-view} shows contour of the discontinuous pulse in the space-time mesh at the final refinement state. \figref{fig:case3-adref-initial-final-plot} shows the cross-section of the pulse at $t=0$ and at $t=1$. The interior of the pulse has bigger elements than the boundary of the pulse where the discontinuity lies. As mentioned before, the solution quality near the discontinuity is restricted by the underlying continuous Galerkin method which is not ideal at approximating discontinuities. This produces overshoot and undershoot near the discontinuity which results in higher residual and eventually high refinement near the discontinuity. \figref{fig:case3-adref-final-state-xy-slice} shows a 2D $x-y$ slice and \figref{fig:case3-adref-final-state-yt-slice} shows a 2D $y-t$ slice of the final refined mesh. Once again the mesh size varies greatly throughout the domain.

% \end{document}

==> sections/5_conclusions.tex <==
% \documentclass[../main.tex]{subfiles}
% \begin{document}
%################################# SECTION ##########################################
%################################# SECTION ##########################################
%################################# SECTION ##########################################
%################################# SECTION ##########################################

\section{Conclusions}\label{sec:conclusion}
In this work we considered a coupled-space-time finite element formulation of the time-dependent advection-diffusion equation using continuous Galerkin method. Such an operator can be cast as a generalized advection-diffusion equation in the space-time domain. Due to the non-dissipative nature of the advection operator, the discrete problem corresponding to these equations may become unstable. To overcome this lack of stability of the discrete variational problem, we formulate an analogue of the Galerkin/least square (GLS) stabilization method in space-time. We show that the GLS-type regularization results in a stable discrete variational problem. We subsequently prove a priori error estimates; and also present a residual based a posteriori error estimate that is used to achieve adaptive refinement in space-time. 

We test our method on various numerical examples such as the heat equation (smooth solution) and the advection-diffusion equation  (both smooth and non-smooth solution). An interesting feature of the space-time solution is that the solution does not suffer any phase error. Also when approximating a discontinuous solution, the space-time method display considerably less oscillations compared to a sequential method of similar accuracy (Crank-Nicolson method). When coupled with an adaptive mesh refinement strategy, both smooth and discontinuous fields can be approximated closely and can even model no-loss solution in the presence of negligible diffusion.

Potential future work include extension to other stabilization techniques such as the streamline upwind Petrov Galerkin method and the variational multiscale method. In addition, nonlinear equations pose significantly different challenges compared to linear PDEs, therefore nonlinear operators such as the Cahn-Hilliard system or the Navier-Stokes equation need to be considered and analyzed with such a formulation. Furthermore, all the examples in this paper were obtained using 3D space-time (i.e., 2D + time) meshes, thus another avenue of future works include extension of the computational meshes to four-dimensions.



% \end{document}

==> sections/6_16_ad_case3_problem_def_schematic.tex <==
\begin{figure}[!htb]
    \centering
    \begin{minipage}[t]{.49\textwidth}
      \centering
      \includegraphics[width=0.99\linewidth]{results_data/ts_case3_ad_sharpic_uniref/k_0_mesh_128/case3_mesh128_at_t_0.png}
      \caption{Initial condition for the pure advection case}
      \label{fig:ad-case3-initial-condition-contour}
    \end{minipage}
    % \hskip 5pt
    % \begin{minipage}[t]{.49\textwidth}
    %   \centering
    %   \frame{\includegraphics[width=0.99\linewidth]{results_data/ts_case2_ad_smoothic_uniref/k_1e-4_mesh_128/at_t_1_line_for_plot.png}}
    %   \caption{'AB' is the line that coincides with the direction of the advection velocity at the (theoretical) center of the pulse}
    %   \label{fig:ad-case2-plot-line-sketch}
    % \end{minipage}
\end{figure}

==> sections/6_appendices.tex <==
%\documentclass[../main.tex]{subfiles}
%\begin{document}
%################################# SECTION ##########################################
%################################# SECTION ##########################################
%################################# SECTION ##########################################
%################################# SECTION ##########################################

\appendix
%\input{sections/6_proofs.tex}
\input{sections/6_proofs_new.tex}
%\input{sections/6_appendices_stability_higher_order.tex}
%\input{sections/6_appendices_stab_no_stab.tex}
%\input{sections/6_appendices_dispersion.tex}
%\end{document}

==> sections/6_appendices_dispersion.tex <==
\section{Dispersion plots}\label{sec:dispersion-study}
\begin{figure}[!htb]
    \centering
    % Space-time solution with uniform mesh of $128^3$\\
    % \begin{minipage}[t]{.49\textwidth}
    %   \centering
    %   $\kappa = 10^{-2}$
    % \end{minipage}
    % \begin{minipage}[t]{.49\textwidth}
    %   \centering
    %   $\kappa = 10^{-4}$
    % \end{minipage}
    % \\
    \begin{minipage}[t]{.75\textwidth}
      \centering
      \begin{tikzpicture}
      \begin{axis}[
          width=0.99\linewidth, % Scale the plot to \linewidth
          %grid=major, % Display a grid
          %grid style={line width=.1pt, draw=gray!50}, % Set the style
          xlabel=$s$, % Set the labels
          ylabel=$u$,
          legend cell align={left},
          legend style={at={(1,1)},anchor=north east,legend columns=1}, % Put the legend below the plot
          x tick label style={rotate=0,anchor=north} % Display labels sideways
        ]
        \addplot+ [color=blue,dashed,mark=none]
        table[x expr={\thisrow{arc_length}},y expr={\thisrow{u}},col sep=comma]{results_data/case_2_ad_smoothic_dispersion/t0_ref_lvl_6.csv};
        \addplot+ [mark=none]
        table[x expr={\thisrow{arc_length}},y expr={\thisrow{u}},col sep=comma]{results_data/case_2_ad_smoothic_dispersion/t1_ref_lvl_3.csv};
        \addplot+ [mark=none]
        table[x expr={\thisrow{arc_length}},y expr={\thisrow{u}},col sep=comma]{results_data/case_2_ad_smoothic_dispersion/t1_ref_lvl_4.csv};
        \addplot+ [mark=none]
        table[x expr={\thisrow{arc_length}},y expr={\thisrow{u}},col sep=comma]{results_data/case_2_ad_smoothic_dispersion/t1_ref_lvl_5.csv};
        \addplot+ [mark=none]
        table[x expr={\thisrow{arc_length}},y expr={\thisrow{u}},col sep=comma]{results_data/case_2_ad_smoothic_dispersion/t1_ref_lvl_6.csv};
        \legend{
        \scriptsize{$t=0$},
        \scriptsize{$t=1$, $8^3$ mesh},
        \scriptsize{$t=1$, $16^3$ mesh},
        \scriptsize{$t=1$, $32^3$ mesh},
        \scriptsize{$t=1$, $64^3$ mesh}}
      \end{axis}
    \end{tikzpicture}
    \end{minipage}
\end{figure}

==> sections/6_appendices_stab_no_stab.tex <==
\section{Comparison between stabilized and non-stabilized solutions}\label{sec:app:comp-stab-no-stab}
\begin{figure}[!htb]
    \centering
    % Space-time solution with uniform mesh of $128^3$\\
    % \begin{minipage}[t]{.49\textwidth}
    %   \centering
    %   $\kappa = 10^{-2}$
    % \end{minipage}
    % \begin{minipage}[t]{.49\textwidth}
    %   \centering
    %   $\kappa = 10^{-4}$
    % \end{minipage}
    % \\
    \begin{minipage}[t]{.75\textwidth}
      \centering
      \begin{tikzpicture}
      \begin{axis}[
          width=0.99\linewidth, % Scale the plot to \linewidth
          %grid=major, % Display a grid
          %grid style={line width=.1pt, draw=gray!50}, % Set the style
          xlabel=$s$, % Set the labels
          ylabel=$u$,
          legend cell align={left},
          legend style={at={(1,1)},anchor=north east,legend columns=1}, % Put the legend below the plot
          x tick label style={rotate=0,anchor=north} % Display labels sideways
        ]
        \addplot+ [color=blue,dashed,mark=none]
        table[x expr={\thisrow{"arc_length"}},y expr={\thisrow{"u"}},col sep=comma]{results_data/case_2_ad_smoothic_stab_no_stab_comparison/case2_stab_both_lvl5_t0.csv};
        \addplot+ [thick,mark=none]
        table[x expr={\thisrow{"arc_length"}},y expr={\thisrow{"u"}},col sep=comma]{results_data/case_2_ad_smoothic_stab_no_stab_comparison/case2_stab_none_lvl5_t1.csv};
        \addplot+ [thick,mark=none]
        table[x expr={\thisrow{"arc_length"}},y expr={\thisrow{"u"}},col sep=comma]{results_data/case_2_ad_smoothic_stab_no_stab_comparison/case2_stab_space_lvl5_t1.csv};
        \addplot+ [thick,mark=none]
        table[x expr={\thisrow{"arc_length"}},y expr={\thisrow{"u"}},col sep=comma]{results_data/case_2_ad_smoothic_stab_no_stab_comparison/case2_stab_time_lvl5_t1.csv};
        \addplot+ [thick,mark=none]
        table[x expr={\thisrow{"arc_length"}},y expr={\thisrow{"u"}},col sep=comma]{results_data/case_2_ad_smoothic_stab_no_stab_comparison/case2_stab_both_lvl5_t1.csv};
        \legend{
        \small{$t=0$},
        \small{$t=1$, No-stab},
        \small{$t=1$, Stab-spatial},
        \small{$t=1$, Stab-time},
        \small{$t=1$, Stab-both}
        }
      \end{axis}
    \end{tikzpicture}
    \end{minipage}
    \caption{Mesh size: $32^3$}
\end{figure}


\begin{figure}[!htb]
    \centering
    % Space-time solution with uniform mesh of $128^3$\\
    % \begin{minipage}[t]{.49\textwidth}
    %   \centering
    %   $\kappa = 10^{-2}$
    % \end{minipage}
    % \begin{minipage}[t]{.49\textwidth}
    %   \centering
    %   $\kappa = 10^{-4}$
    % \end{minipage}
    % \\
    \begin{minipage}[t]{.49\textwidth}
      \centering
      \begin{tikzpicture}
      \begin{axis}[
          width=0.99\linewidth, % Scale the plot to \linewidth
          %grid=major, % Display a grid
          %grid style={line width=.1pt, draw=gray!50}, % Set the style
          xlabel=$s$, % Set the labels
          ylabel=$u$,
          legend cell align={left},
          legend style={at={(1,1)},anchor=north east,legend columns=1}, % Put the legend below the plot
          x tick label style={rotate=0,anchor=north} % Display labels sideways
        ]
        \addplot+ [color=blue,dashed,mark=none]
        table[x expr={\thisrow{"arc_length"}},y expr={\thisrow{"u"}},col sep=comma]{results_data/case_2_ad_smoothic_stab_no_stab_comparison/case2_stab_both_lvl6_t0.csv};
        \addplot+ [thick,mark=none]
        table[x expr={\thisrow{"arc_length"}},y expr={\thisrow{"u"}},col sep=comma]{results_data/case_2_ad_smoothic_stab_no_stab_comparison/case2_stab_none_lvl6_t1.csv};
        \addplot+ [thick,mark=none]
        table[x expr={\thisrow{"arc_length"}},y expr={\thisrow{"u"}},col sep=comma]{results_data/case_2_ad_smoothic_stab_no_stab_comparison/case2_stab_space_lvl6_t1.csv};
        \addplot+ [thick,mark=none]
        table[x expr={\thisrow{"arc_length"}},y expr={\thisrow{"u"}},col sep=comma]{results_data/case_2_ad_smoothic_stab_no_stab_comparison/case2_stab_time_lvl6_t1.csv};
        \addplot+ [thick,mark=none]
        table[x expr={\thisrow{"arc_length"}},y expr={\thisrow{"u"}},col sep=comma]{results_data/case_2_ad_smoothic_stab_no_stab_comparison/case2_stab_both_lvl6_t1.csv};
        \legend{
        \small{$t=0$},
        \small{$t=1$, No-stab},
        \small{$t=1$, Stab-spatial},
        \small{$t=1$, Stab-time},
        \small{$t=1$, Stab-both}
        }
      \end{axis}
    \end{tikzpicture}
    \end{minipage}
    \caption{Mesh size: $64^3$}
\end{figure}
\clearpage

==> sections/6_appendices_stability_higher_order.tex <==
%\documentclass[../main.tex]{subfiles}
%\begin{document}

%\end{document}

==> sections/6_proofs.tex <==
\section{Proofs for Section \ref{sec:math-formulation}}
%\begin{lemma}
%The bilinear form \eqref{def:discrete-bilinear-form-truncated} is uniformly bounded on $V_h\times V_h$, i.e.,
%\begin{align}
%    |\bformh(\vh,\wh)|\leq\mu_b\normH{\vh}{\Omega}\normH{\wh}{\Omega}
%\end{align}
%\end{lemma}
\subsection{Lemma \ref{lemma:boundedness} (Boundedness)}\label{sec:proof-boundeness}
\begin{proof}[Proof of Lemma \ref{lemma:boundedness}]
We consider each of the inner product in \eqref{def:discrete-bilinear-form-truncated} and bound them from above.
\begin{enumerate}
%1
    \item The first term $(\vht,\wh)$ is first integration by parts and then each of the resulting term is estimated from below:
    \begin{align*}
        |(\vht,\wh)| &= \left|\intTimeSpace\vht\wh dUdt \right| = \left|-\intTimeSpace\vh\wh_t dUdt + \int_{\bft}\vh\wh dS\right|\\
        &\leq\left|-\intTimeSpace\vh\wh_t dUdt\right| + \left|\int_{\bft}\vh\wh dS\right|\\
        &\leq \normL\vh\Omega\normL{\wh_t}{\Omega} + \normL\vh\bft\normL\wh\bft
    \end{align*}
%2
    \item Each of the next six terms in \eqref{def:discrete-bilinear-form-truncated} can be easily bounded from above by applying Cauchy-Schwarz inequality
    \begin{align*}
        |(\adv\cdot\grad\vh,\wh)|\leq\normL{\adv\cdot\grad\vh}{\Omega}\normL{\wh}{\Omega}\leq |\adv|\normL{\grad\vh}{\Omega}\normL\wh\Omega
    \end{align*}
%3
    \item
    \begin{align*}
        |(\kappa\grad\vh,\grad\wh)|\leq \kappa\normL{\grad\vh}{\Omega}\normL{\grad\wh}{\Omega}
    \end{align*}
%4
    \item
    \begin{align*}
        |\glspar(\vht,\wh_t)|\leq \glspar\normL{\vht}{\Omega}\normL{\wh_t}{\Omega}
    \end{align*}
%5
    \item
    \begin{align*}
        |\glspar(\adv\cdot\grad\vh,\adv\cdot\grad\wh)|\leq \glspar\left(\normL[\infty]{\adv}{\Omega}\normL{\grad\vh}{\Omega}\right)\left(\normL[\infty]{\adv}{\Omega}\normL{\grad\wh}{\Omega}\right)
    \end{align*}
%6
    \item
    \begin{align*}
        | \glspar(\vht,\adv \cdot \grad \wh) | \leq \glspar \normL{\vht}{\Omega} \normL[\infty]{\adv}{\Omega} \normL{\grad \wh}{\Omega}
    \end{align*}
%7
    \item
    \begin{align*}
        |\glspar(\adv\cdot\grad\vh,\wh_t)|\leq \glspar\normL[\infty]{\adv}{\Omega}\normL{\grad \vh}{\Omega}\normL{\wh_t}{\Omega}
    \end{align*}
%8
    \item While trying to put an upper bound to $\glspar\kappa(\grad\vht,\grad\wh)$, we note that $\grad\vht$ is a second derivative on $\vh$ with respect to both space and time. We estimate this term by only the spatial derivatives through the use of the inverse estimates.
    \begin{align*}
        \normL{\grad\vht}{\Omega} 
        = \intOmega \left[|\grad \vht|^2 \right]d\Omega 
        = \intOmega \left[\sum_{i=1}^{\nsd}|{\vh}_{t x_i}|^2 \right]d\Omega 
        =  \sum_{i=1}^{\nsd}\left[\intOmega|{\vh}_{t x_i}|^2 d\Omega \right]
        %= \sum_{i=1}^{\nsd}\normL{{\vh}_{t x_i}}{\Omega}
    \end{align*}
    The integratioin over $\Omega $ is equal to the sum of integration over all the individual elements in the mesh, i.e.,
    \begin{align*}
        \sum_{i=1}^{\nsd}\left[\intOmega|{\vh}_{t x_i}|^2 d\Omega \right]
        = \sum_{i=1}^{\nsd} \sum_{K\in\mesh} \left[\int_{K}|{\vh}_{t x_i}|^2 dK \right]
        = \sum_{i=1}^{\nsd} \sum_{K\in\mesh} \normL{{\vh}_{t x_i}}{K}^2
    \end{align*}
    There exist a positive constant $\invCoefOne$ such that
    \begin{align*}
        \normL{{\vh}_{t x_i}}{K}^2
        \leq \invCoefOne^2 h^{-2}\normL{{\vh}_{x_i}}{K}^2 \textrm{ for }i = 1,2,...,\nsd
    \end{align*}
    Therefore we have,
    \begin{align*}
        \normL{\grad\vht}{\Omega}  &\leq
        \sum_{i=1}^{\nsd} \sum_{K\in\mesh} \invCoefOne^2 h^{-2}\normL{{\vh}_{x_i}}{K}^2
         = \invCoefOne h^{-2}\sum_{i=1}^{\nsd} \sum_{K\in\mesh}\left[\int_{K}|{\vh}_{x_i}|^2 dK \right]\\
         &= \invCoefOne^2 h^{-2}\sum_{i=1}^{\nsd} \left[\intOmega|{\vh}_{x_i}|^2 d\Omega \right]
         = \invCoefOne^2 h^{-2}\intOmega \left[\sum_{i=1}^{\nsd}|{\vh}_{x_i}|^2 \right]d\Omega
         = \invCoefOne^2 h^{-2}\normL{\grad \vh}{\Omega}
    \end{align*}
    So finally applying Cauchy Schwarz inequality on $\glspar\kappa(\grad\vht,\grad\wh)$, we have,
    \begin{align*}
        |\glspar\kappa(\grad\vht,\grad\wh)| &\leq \glspar\kappa\normL{\grad\vht}{\Omega}\normL{\grad\wh}{\Omega}
        \leq \glspar\kappa\invCoefOne h^{-1}\normL{\grad \vh}{\Omega}\normL{\grad\wh}{\Omega}
        % &\leq \glspar\kappa \sum_{K\in\mathcal{K_h}}
        % &\leq \glspar\kappa\invCoefOne^2\normL{\grad\vh}{\Omega}\normL{\grad\wh}{\Omega}
    \end{align*}
%9
    \item The next term $\glspar\kappa(\grad\vh,\grad\wh_t)$ similar to the previous one and can be estimated in the same way
    \begin{align*}
        |\glspar\kappa(\grad\vh,\grad\wh_t)| \leq \glspar\kappa\normL{\grad\wh}{\Omega}\normL{\grad\wh_t}{\Omega}
        \leq \glspar\kappa\invCoefOne h^{-1}\normL{\grad\vh}{\Omega}\normL{\grad\wh}{\Omega}
    \end{align*}
\end{enumerate}
Now we combine all these terms using Cauchy's inequality and get,
\begin{align} \label{est:boundedness-second-last-result}
    |\bformh(\vh,\wh)| \leq \left[ X(\vh) \right]^{\frac{1}{2}}\left[ Y(\wh) \right]^{\frac{1}{2}}
\end{align}
where, $X(\vh)$ and $Y(\wh)$ are as follows,
\begin{align*}
    X(\vh) & = \left[
    \glspar^{-1}\normL{\vh}{\Omega}^2 + \normL{\vh}{\bft}^2 + 
    2\glspar\normL{\vht}{\Omega}^2 + \left((1+2\glspar)\normL[\infty]{\adv}{\Omega}^2 + \left(\frac{\glspar}{h}\right)^2\invCoefOne^2 + 2\kappa \right)\normL{\grad\vh}{\Omega}^2
    \right]^{\frac{1}{2}}
    \\
    Y(\wh) & = \left[
    \normL{\wh}{\bft}^2 + 
    (1+3\glspar)\normL{\wh_t}{\Omega}^2 + \left(2\glspar\normL[\infty]{\adv}{\Omega}^2 + \left(\frac{\glspar}{h}\right)^2\invCoefOne^2 + 2(\kappa+\glspar) \right)\normL{\grad\wh}{\Omega}^2
    \right]^{\frac{1}{2}}
\end{align*}
The inequality \ref{est:boundedness-second-last-result} can then be estimated as
\begin{align}
    |\bformh(\vh,\wh)| \leq \mu_b \normVstar{\vh}\normV{\wh}
\end{align}
\end{proof}

\subsection{Lemma \ref{lemma:coercivity-stability} (Coercivity)}\label{sec:proof-coercivity}
\begin{proof}[Proof of Lemma \ref{lemma:coercivity-stability}]
	From \eqref{def:discrete-bilinear-form-truncated} we have,
	\begin{align*}
		\begin{split}
			\bformh(\vh,\vh) &= 
			\int_0^T\int_U \Big[
			\vh\vht
			+\vh(\adv\cdot\grad\vh)
			+\kappa\modulus{\grad\vh}^2
			+\glspar(\vht)^2
			+2\glspar\vht(\adv\cdot\grad\vh) \\
			&\quad+2\glspar\kappa(\grad\vh\cdot\grad\vht)
			+\glspar(\adv\cdot\grad\vh)^2
			\Big] dUdt\\
			&= 
			\int_0^T\int_U \Big[
			\vh\vht
			+2\glspar\kappa(\grad\vh\cdot\grad\vht)
			+\vh(\adv\cdot\grad\vh)
			+\kappa\modulus{\grad\vh}^2
			+\glspar(\vht)^2\\
			&\quad+2\glspar\vht(\adv\cdot\grad\vh)
			+\glspar(\adv\cdot\grad\vh)^2
			\Big] dUdt.
		\end{split}\\
	\end{align*}
	% The first term is
	% \begin{align*}
		%     \intTimeSpace\vh\vht = \intTimeSpace \frac{1}{2}\frac{\partial}{\partial t}(\vh)^2 dUdt = \frac{1}{2}\left(\normL\vh\bft^2 - \normL\vh\bit^2 \right) = \frac{1}{2}\normL\vh\bft^2
		% \end{align*}
	% The second term can be similarly written as
	% \begin{align*}
		%     \intTimeSpace \glspar\kappa (\grad\vh\cdot\grad\vht + \grad\vht\cdot\grad\vh)dUdt = \glspar\kappa\intTimeSpace \frac{\partial}{\partial t}(\modulus{\grad\vh}^2)dUdt = \glspar\kappa\normL{\grad\vh}{\bft}^2
		% \end{align*}
	The first two terms in the above expression are related to the trace of the function $\vh$ restricted to the final time boundary:
	\begin{align*}
		\intTimeSpace \vh\vht
		+2\glspar\kappa(\grad\vh\cdot\grad\vht)dUdt &= 
		\intTimeSpace \left[\frac{\partial}{\partial t}\left(\frac{(\vh)^2}{2}\right) + \glspar\kappa\frac{\partial}{\partial t}\left(\grad\vh\cdot\grad\vh\right)\right] dUdt\\
		&= \frac{1}{2}\left(\normL\vh\bft^2 - \normL\vh\bit^2 \right) + \glspar\kappa(\normL{\grad\vh}{\bft}^2-\normL{\grad\vh}{\bit}^2)\\
		&= \frac{1}{2}\normL\vh\bft^2+ \glspar\kappa\normL{\grad\vh}{\bft}^2.
	\end{align*}
	Because of the divergence-free velocity field, the third term evaluates to zero:
	\begin{align*}
		\intTimeSpace\vh(\adv\cdot\grad\vh)dUdt &= \intTimeSpace \adv\cdot(\vh\grad\vh) = \frac{1}{2}\intTimeSpace \adv\cdot\grad(\vh)^2 = \frac{1}{2}\intTimeSpace \grad\cdot(\adv(\vh)^2)\\  &=\frac{1}{2}\int_0^T\int_{\partial U}\hat{n}\cdot(\adv(\vh)^2) dSdt = 0
	\end{align*}
	since $\vh=0$ on $\partial U$. Finally, the last four terms can be taken collectively,
	\begin{align*}
		S &= \intTimeSpace\left[
		\kappa\modulus{\grad\vh}^2
		+\glspar(\vht)^2
		+2\glspar\vht(\adv\cdot\grad\vh)
		+\glspar(\adv\cdot\grad\vh)^2\right] dUdt\\
		&= \intTimeSpace\left[\kappa\sum_{i=1}^{n}({\vh}_{x_i})^2 + \glspar(\vht)^2 + 2\glspar\sum_{i=1}^{n}\vht\advcomp{i}{\vh}_{x_i} + \glspar\left(\sum_{i=1}^{n}(\advcomp{i}{\vh}_{x_i})^2+\sum_{\substack{i,j=1 \\ j\neq i}}^{n}\advcomp{i}\advcomp{j}{\vh}_{x_i}{\vh}_{x_j}\right)\right]dUdt\\
		&=\intTimeSpace\left[ \sum_{i=1}^n(\kappa+\glspar \advcomp{i}^2)({\vh}_{x_i})^2 + \glspar(\vht)^2 + \sum_{i=1}^n2\glspar\advcomp{i}\vht{\vh}_{x_i}+\sum_{\substack{i,j=1 \\ j\neq i}}^n\advcomp{i}\advcomp{j}{\vh}_{x_i}{\vh}_{x_j} \right]dUdt\\
		&=\intTimeSpace \left(\gradst\vh\cdot\mmat{M}\cdot\gradst\vh\right)dUdt,
	\end{align*}
	where $\gradst\vh$ is defined in \ref{operator:grad-st}, and $\mmat{M}$ is defined as,
	\begin{align}
		\mmat{M}=
		\begin{bmatrix}
			\kappa+\glspar \advcomp{1}^2 & \glspar\advcomp{1}\advcomp{2} &\cdots & \glspar\advcomp{1}\advcomp{n} & \glspar\advcomp{1} \\
			\glspar\advcomp{1}\advcomp{2} & \kappa+\glspar \advcomp{2}^2 &\cdots & \glspar\advcomp{2}\advcomp{n} & \glspar\advcomp{2}\\
			\vdots & \vdots & \ddots & \vdots & \vdots\\
			\glspar\advcomp{1}\advcomp{n} & \glspar\advcomp{2}\advcomp{n} & \cdots & \kappa+\glspar\advcomp{n}^2 & \glspar\advcomp{n} \\
			\glspar\advcomp{1} & \glspar\advcomp{2} & \cdots & \glspar\advcomp{n} & \glspar
		\end{bmatrix}_{(n+1)\times(n+1)}.
	\end{align}
	The matrix $\mmat{M}$ plays a role that is similar to the $\mmat{A}$ matrix defined in equation ~\ref{expr:ellipticity-matrix-original}. For $\nsd = 2$, the eigenvalues of $\mmat{M}$ are
	\begin{align*}
		\lambda_1 &= k,\\
		\lambda_2 &= \frac{1}{2}\left[k + \glspar (1 + |\adv|^2) - \sqrt{[k + \glspar (1 + |\adv|^2)]^2 - 4\kappa\glspar}\right],\\
		\lambda_3 &= \frac{1}{2}\left[k + \glspar (1 + |\adv|^2) + \sqrt{[k + \glspar (1 + |\adv|^2)]^2 - 4\kappa\glspar}\right].
	\end{align*}
	The matrix $\mmat{M}$ is symmetric and positive definite, thus its minimum eigenvalue is greater than zero. Thus for any vector $y\in\mathbb{R}^{n+1}$, we have $\mvec{y}^T\mmat{M}\mvec{y}>\glspar |y|^2>0$. Therefore,
	\begin{align*}
		S \geq \intTimeSpace \glspar |\mvec{D}\vh|^2dUdt = \glspar\normL{\gradst\vh}{\Omega}^2.
	\end{align*}
	Putting it all together,
	\begin{align*}
		\bformh(\vh,\vh) &\geq \frac{1}{2}\normL\vh\bft^2+ \glspar\kappa\normL{\grad\vh}{\bft}^2 + \glspar\normL{\gradst \vh}{\Omega}\\
		&\geq \frac{1}{2}\normL\vh\bft^2 + \glspar\normL{\gradst \vh}{\Omega}\\
		&= \frac{1}{2}\normL\vh\bft^2 + \glspar\left(\normL{\grad \vh}{\Omega} + \normL{\vht}{\Omega}\right)\\
		&=\mu_c\normV{\vh},
	\end{align*}
	where $0\leq\mu_c\leq 1$.
\end{proof}

%\section{Stability: higher order basis function}
\subsection{Proof of Lemma \ref{lemma:coercivity-stability} when higher order basis functions are used}\label{sec:proof-coercivity-higher-order}
When higher order basis functions are used, the stability of the discrete problem \eqref{def:discrete-variational-form} can be proved in a simpler way using a different norm. We have, from the left hand side of equation ~\eqref{eq:gls-abstract},
\begin{align}
	\bformh(\vh,\wh) &= (\mathscr{L}\vh, \wh) + \glspar(\mathscr{L}\vh,\mathscr{L}\wh)\\
	&= (\vht,\wh) + (\adv\cdot\grad\vh, \wh) + (\kappa\grad\vh,\grad\wh)\\
	&\qquad +\glspar \big([\vht+\adv\cdot\grad\vh-\kappa\laplacian\vh],[\wh_t+\adv\cdot\grad\wh-\kappa\laplacian\wh]\big)
\end{align}
Therefore,
\begin{align*}
	\bformh(\vh,\vh) &= (\mathscr{L}\vh, \vh) + \glspar(\mathscr{L}\vh,\mathscr{L}\vh)\\
	&= (\vht,\vh) + (\adv\cdot\grad\vh, \vh) + (\kappa\grad\vh,\grad\vh)\\
	&\qquad +\glspar \big([\vht+\adv\cdot\grad\vh-\kappa\laplacian\vh],[\vht+\adv\cdot\grad\vh-\kappa\laplacian\vh]\big)\\
	&= \intTimeSpace \Big[\vh\vht + \vh(\adv\cdot\grad\vh) + \kappa(\grad\vh\cdot\grad\vh)\\
	&\qquad\qquad\qquad\qquad\qquad + \glspar(\vht+\adv\cdot\grad\vh-\kappa\laplacian\vh)^2\Big] dUdt\\
	&= \intTimeSpace \frac{\partial}{\partial t}\left(\frac{(\vh)^2}{2}\right)dUdt 
	+\intTimeSpace \grad\cdot \left(\frac{\adv(\vh)^2}{2}\right)dUdt + \intTimeSpace \kappa|\grad\vh|^2dUdt\\
	&\quad +\intTimeSpace \glspar(\vht+\adv\cdot\grad\vh-\kappa\laplacian\vh)^2 dUdt\\
	&= \frac{1}{2}\left(\normL\vh\bft^2 - \normL\vh\bit^2 \right) + \frac{1}{2}\int_0^T\int_{\partial U}\hat{n}\cdot(\adv(\vh)^2) dSdt + \kappa\normL{\grad\vh}{\Omega}^2\\ &\qquad+\intTimeSpace\glspar\{(\vht+\adv\cdot\grad\vh)-\kappa\laplacian\vh\}^2 dUdt\\
	&= \left(\frac{1}{2}\normL\vh\bft^2 - 0\right)+ 0  + \kappa\normL{\grad\vh}{\Omega}^2\\
	&\qquad +\intTimeSpace \glspar \left[  (\vht+\adv\cdot\grad\vh)^2 +(\kappa\laplacian\vh)^2 -2(\vht+\adv\cdot\grad\vh)(\kappa\laplacian\vh) \right]dUdt\\
	&= \frac{1}{2}\normL\vh\bft^2 + \kappa\normL{\grad\vh}{\Omega}^2 + \normL{\glspar(\vht+\adv\cdot\grad\vh)}{\Omega}^2 + \glspar\kappa^2\normL{\laplacian\vh}{\Omega} \\
	&\qquad -\intTimeSpace \glspar \kappa\left[2\vht\laplacian\vh \right]dUdt -\intTimeSpace \glspar\kappa \left[ 2(\adv\cdot\grad\vh)(\laplacian\vh) \right]dUdt
\end{align*}
The last two integrals can now be examined separately. The first one of them can be evaluated as
\begin{align*}
	-\intTimeSpace \glspar \kappa\left[2\vht\laplacian\vh \right]dUdt
	&= \intTimeSpace\glspar\kappa(2\grad\vht\cdot\grad\vh) dUdt
	= \intTimeSpace\glspar\kappa\frac{\partial}{\partial t}|\grad\vh|^2 dUdt\\
	&= \glspar\kappa(\normL{\grad\vh}{\bft}^2-\normL{\grad\vh}{\bit}^2)
	= \glspar\kappa\normL{\grad\vh}{\bft}^2
\end{align*}
And the very last integral can be estimated with the help of inverse estimates,
\begin{align*}
	-\intTimeSpace \glspar\kappa \left[ 2(\adv\cdot\grad\vh)(\laplacian\vh) \right]dUdt 
	&= -2\glspar\kappa(\adv\cdot\grad\vh,\laplacian\vh) \\
	&\geq -2\glspar\kappa|(\adv\cdot\grad\vh,\laplacian\vh)|\\
	&\geq -2\glspar\kappa \normL[\infty]{\adv}{\Omega}\normL{\grad\vh}{\Omega} C h^{-1}\normL{\grad\vh}{\Omega}\\
	&= - 2C h^{-1}\glspar\kappa\normL[\infty]{\adv}{\Omega}\normL{\grad\vh}{\Omega}
\end{align*}
Therefore
\begin{align}
	\bformh(\vh,\vh) &\geq 
	\frac{1}{2}\normL\vh\bft^2 + \kappa\normL{\grad\vh}{\Omega}^2 + \normL{\glspar(\vht+\adv\cdot\grad\vh)}{\Omega}^2 + \glspar\kappa^2\normL{\laplacian\vh}{\Omega}\\
	& \qquad + \glspar\kappa\normL{\grad\vh}{\bft}^2 - 2Ch^{-1}\glspar\kappa\normL[\infty]{\adv}{\Omega}\normL{\grad\vh}{\Omega}\\
	&=\frac{1}{2}\normL\vh\bft^2 + \glspar\kappa\normL{\grad\vh}{\bft}^2 + \normL{\glspar(\vht+\adv\cdot\grad\vh)}{\Omega}^2 \\
	&\qquad + (\kappa - 2Ch^{-1}\glspar\kappa\normL[\infty]{\adv}{\Omega})\normL{\grad\vh}{\Omega}+ \glspar\kappa^2\normL{\laplacian\vh}{\Omega}
\end{align}

\subsection{Lemma \ref{lemma:interp-estimate-in-Vh}} \label{proof:interp-estimate-vh}
\begin{proof}
We have
\begin{align*}
\normV{v-\interp{v}}^2  = \left[\normVExpanded{v-\interp{v}}\right].
\end{align*}
Each of the individual norms appearing on the right hand side can be estimated using the estimates \eqref{estimate:sobolev-interp-boundary-L2}, \eqref{estimate:sobolev-interp-grad-L2} and \eqref{estimate:sobolev-interp-time-der-L2} respectively. So, we have
% We proceed by estimating each of the norms appearing on the right hand side by the seminorm of $v$ in $H^m(\stDom)$
% \begin{itemize}
%     \item The first norm is a norm on the final time boundary. We apply the scaled trace inequlaity from \ref{estimate:scaled-trace-inequality} to estimate this norm.
%     \begin{align}
%         \frac{1}{2}\normL{v-\interp{v}}{\bft}^2 &
%         \leq \frac{1}{2}\normL{v-\interp{v}}{\partial \stDom}^2 \\
%         & = \frac{1}{2}\sum_{\substack{k\in\mesh \\ \partial K \cap \partial \stDom}}\normL{v-\interp{v}}{\partial K \cap \partial \stDom}^2\\
%         &\leq \frac{1}{2}\traceConstant^2 \left[\sum_{\substack{k\in\mesh}}\left( h_K^{-1}\normL{v-\interp{v}}{K}^2 + h_K\normH[1]{v-\interp{v}}{K}^2 \right)  \right]\\
%         & \leq \frac{1}{2}\traceConstant^2 \left[ \shapeRegularConst h^{-1} \normL{v-\interp{v}}{\stDom}^2 + h \normH[1]{v-\interp{v}}{\stDom}^2 \right]\\
%         & \leq \frac{1}{2}\traceConstant^2 \left[ \shapeRegularConst h^{-1} \approxConstant^2 h^{2(k+1-0)}|v|_{H^{k+1}(\stDom)}^2  + h\approxConstant^2 h^{2(k+1-1)}|v|_{H^{k+1}(\stDom)}^2  \right]\\
%         & = \frac{1}{2}\traceConstant^2 \left[ \shapeRegularConst \approxConstant^2 h^{2k+1} + \approxConstant^2 h^{2k+1}\right]|v|_{H^{k+1}(\stDom)}^2\\
%         & = \frac{1}{2}\traceConstant^2 \approxConstant^2  \left( \shapeRegularConst + 1\right)h^{2k+1}|v|_{H^{k+1}(\stDom)}^2
%     \end{align}
%     \item The next two terms are estimated more directly by applying the result \ref{estimate:sobolev-approximation}
%     \begin{align*}
%         \gamma \normL{\grad(v-\interp{v})}{\stDom} \leq \gamma \approxConstant^2 h^{2(k+1-1)}|v|_{H^{k+1}}^2
%         = \gamma \approxConstant^2 h^{2k}|v|_{H^{k+1}}^2
%     \end{align*}
%     and 
%     \begin{align*}
%         \gamma \normL{(v-\interp{v})_t}{\stDom} \leq \gamma \approxConstant^2 h^{2(k+1-1)}|v|_{H^{k+1}}^2
%         = \gamma \approxConstant^2 h^{2k}|v|_{H^{k+1}}^2
%     \end{align*}
% \end{itemize}
% Finally combining the estimates, we have,
\begin{align*}
\normV{v-\interp{v}}^2 &\leq
\left( \frac{1}{2}{\approxConstant}_{\Gamma}^2 h^{2k+1}  +\gamma {\approxConstant}_1^2 h^{2k} + \gamma {\approxConstant}_1^2 h^{2k} \right)|v|_{H^{k+1}}^2\\
& = \left( \frac{1}{2}{\approxConstant}_{\Gamma}^2 h + 2\gamma \approxConstant^2\right)h^{2k}|v|_{H^{k+1}}^2\\
& = C^2 h^{2k}\seminormH[k+1]{v}{\stDom}^2,
\end{align*}
which then yields the required estimate.
\end{proof}

\subsection{Theorem \ref{theorem:a-priori-estimate} (A priori error estimate)} \label{sec:proof-a-priori}
\begin{proof}[Proof of Theorem \ref{theorem:a-priori-estimate}]
	Define $\er = \vh-v$, $\eh = \vh-\interpolant v$ and $\ei = \interpolant v - v$. These three quantities are related as
	\begin{align}
		\er = \eh + \ei
	\end{align}
	By triangle inequality
	\begin{align}
		\normV{\er} \leq \normV{\eh} + \normV{\ei}
		\label{eq:errors-triangle-ineq}
	\end{align}
	From Lemma \ref{lemma:interp-estimate-in-Vh}, the estimate on $\normV{\ei}$ is already known, i.e.,
	\begin{align}
		\normV{\ei}\leq C_1 h^k|v|_{H^{k+1}(\Omega)}
	\end{align}
	Now we try to estimate $\normV{\eh}$ which will eventually give an estimate of $\normV{\er}$.
	We have
	\begin{align}
		\begin{split}
			\normV{\eh}^2 
			&\leq \bformh(\eh,\eh) = \bformh(\er-\ei,\eh) = \bformh(\er,\eh)-\bform(\ei,\eh) = -\bform(\ei,\eh)\\
			&\leq |\bform(\ei,\eh)|
		\end{split}
		\\
		\begin{split}
			&\leq 
			|(\ei_t,\eh)| + |(\adv\cdot\grad\ei, \eh)| + |(\kappa\grad\ei,\grad\eh)|\\
			&\quad +\glspar|(\ei_t,\eh_t)| + \glspar|(\ei_t,\adv\cdot\grad\eh)|+\glspar|(\grad\ei_t,\kappa\grad\eh)|\\
			&\quad +\glspar|(\adv\cdot\grad\ei,\eh_t)|+\glspar|(\adv\cdot\grad\ei,\adv\cdot\grad\eh)|
			+\glspar|(\kappa\grad\ei,\grad\eh_t)|
		\end{split}
		\label{def:discrete-bilinear-form-for-error}
	\end{align}
	We consider each of the inner products appearing on the right hand side of the above inequality and bound them from above.
	\begin{itemize}
		%1
		\item The first term $(\ei_t,\eh)$ is first integrated by parts and then each of the resulting terms is estimated using the Cauchy-Schwarz inequality:
		\begin{align*}
			|(\ei_t,\eh)| &= \left|\intTimeSpace\ei_t\eh dUdt \right| = \left|-\intTimeSpace\ei\eh_t dUdt + \int_{\bft}\ei\eh dS\right|\\
			&\leq\left|-\intTimeSpace\ei\eh_t dUdt\right| + \left|\int_{\bft}\ei\eh dS\right|\\
			&\leq \normL\ei\Omega\normL{\eh_t}{\Omega} + \normL\ei\bft\normL\eh\bft\\
			&\leq C_{a0}h^{k+1}\seminormH[k+1]{v}{\Omega}(\glspar^{-1}\glspar)\normL{\eh_t}{\Omega} + C_{a\Gamma}h^{k+1}\seminormH[k+1]{v}{\Omega}\normL\eh\bft\\
			&\leq C^{1}\left(\glspar\normL{\eh_t}{\Omega} + \frac{1}{2}\normL\eh\bft\right)h^{k}\seminormH[k+1]{v}{\Omega}
		\end{align*}
		%2
		\item Each of the next six terms in \eqref{def:discrete-bilinear-form-for-error} can be easily bounded from above by applying the Cauchy-Schwarz inequality. We have
		\begin{align*}
			|(\adv\cdot\grad\ei,\eh)| &= |-(\ei,\adv\cdot\grad\eh)|
			\leq\normL{\ei}{\Omega}\normL{\adv\cdot\grad\eh}{\Omega}\\
			&\leq \normL{\ei}{\Omega}\normL[\infty]{\adv}{\Omega}\normL{\grad\eh}{\Omega}\\
			&\leq \normL[\infty]{\adv}{\Omega}C_{a1}h^{k+1}\seminormH[k+1]{v}{\Omega}(\glspar^{-1}\glspar)\normL{\grad\eh}{\Omega}\\
			&\leq C^2\left(\glspar\normL{\grad\eh}{\Omega}\right)h^{k}\seminormH[k]{v}{\Omega}.
		\end{align*}
		%3
		\item The third inner product
		\begin{align*}
			|(\kappa\grad\ei,\grad\eh)|
			&\leq \kappa\normL{\grad\ei}{\Omega}\normL{\grad\eh}{\Omega}\\
			&\leq \kappa C_{a1}h^{k}\seminormH[k+1]{v}{\Omega}\normL{\grad\eh}{\Omega}\\
			&\leq  C_{a1} \left(\kappa\normL{\grad\eh}{\Omega}\right)  h^{k}\seminormH[k+1]{v}{\Omega}
		\end{align*}
		%4
		\item The fourth inner product
		\begin{align*}
			|\glspar(\ei_t,\eh_t)|
			&\leq \glspar\normL{\ei_t}{\Omega}\normL{\eh_t}{\Omega}
			\leq \glspar C_{a1}h^{k}\seminormH[k+1]{v}{\Omega}\normL{\eh_t}{\Omega}
			\leq C_{a1}\left(\glspar\normL{\eh_t}{\Omega}\right)h^{k}\seminormH[k+1]{v}{\Omega}
		\end{align*}
		%5
		\item The fifth inner product
		\begin{align*}
			|\glspar(\adv\cdot\grad\ei,\adv\cdot\grad\eh)|
			&\leq \glspar\left(\normL[\infty]{\adv}{\Omega}\normL{\grad\ei}{\Omega}\right)\left(\normL[\infty]{\adv}{\Omega}\normL{\grad\eh}{\Omega}\right)\\
			&\leq \glspar\left(\normL[\infty]{\adv}{\Omega}C_{a1}h^{k}\seminormH[k+1]{v}{\Omega}\right)\left(\normL[\infty]{\adv}{\Omega}\normL{\grad\eh}{\Omega}\right)\\
			&\leq C^5 \left(\glspar\normL{\grad\eh}{\Omega}\right) h^{k}\seminormH[k+1]{v}{\Omega}
		\end{align*}
		%6
		\item The sixth inner product
		\begin{align*}
			| \glspar(\ei_t,\adv \cdot \grad \eh) | 
			&\leq \glspar \normL{\ei_t}{\Omega} \normL[\infty]{\adv}{\Omega} \normL{\grad \eh}{\Omega}\\
			&\leq \glspar C_{a1}h^{k}\seminormH[k+1]{v}{\Omega} \normL[\infty]{\adv}{\Omega} \normL{\grad \eh}{\Omega}\\
			&\leq C^6 \left(\glspar\normL{\grad \eh}{\Omega}\right) h^{k}\seminormH[k+1]{v}{\Omega}
		\end{align*}
		%7
		\item The seventh inner product
		\begin{align*}
			|\glspar(\adv\cdot\grad\ei,\eh_t)|
			&\leq \glspar\normL[\infty]{\adv}{\Omega}\normL{\grad \ei}{\Omega}\normL{\eh_t}{\Omega}\\
			&\leq \glspar\normL[\infty]{\adv}{\Omega} C_{a1}h^{k}\seminormH[k+1]{v}{\Omega}\normL{\eh_t}{\Omega}\\
			&\leq C^7 \left(\glspar\normL{\eh_t}{\Omega}\right) h^{k}\seminormH[k+1]{v}{\Omega}
		\end{align*}
		%8
		\item While trying to put an upper bound on $\glspar\kappa(\grad\ei_t,\grad\eh)$, we note that $\grad\ei_t$ is a second derivative of $\ei$ with respect to both space and time. We estimate this term by only the spatial derivatives through the use of the inverse estimates.
		\begin{align*}
			\normL{\grad\ei_t}{\Omega} 
			= \intOmega \left[|\grad \ei_t|^2 \right]d\Omega 
			= \intOmega \left[\sum_{i=1}^{\nsd}|\ei_{t x_i}|^2 \right]d\Omega 
			=  \sum_{i=1}^{\nsd}\left[\intOmega|\ei_{t x_i}|^2 d\Omega \right]
			%= \sum_{i=1}^{\nsd}\normL{\ei_{t x_i}}{\Omega}
		\end{align*}
		The integratioin over $\Omega $ is equal to the sum of integration over all the individual elements in the mesh, i.e.,
		\begin{align*}
			\sum_{i=1}^{\nsd}\left[\intOmega|\ei_{t x_i}|^2 d\Omega \right]
			= \sum_{i=1}^{\nsd} \sum_{K\in\mesh} \left[\int_{K}|\ei_{t x_i}|^2 dK \right]
			= \sum_{i=1}^{\nsd} \sum_{K\in\mesh} \normL{\ei_{t x_i}}{K}^2.
		\end{align*}
		There exists a positive constant $\invCoefOne$ such that
		\begin{align*}
			\normL{\ei_{t x_i}}{K}^2
			\leq \invCoefOne^2 h^{-2}\normL{\ei_{x_i}}{K}^2 \textrm{ for }i = 1,2,...,\nsd
		\end{align*}
		Therefore we have,
		\begin{align*}
			\normL{\grad\ei_t}{\Omega}  &\leq
			\sum_{i=1}^{\nsd} \sum_{K\in\mesh} \invCoefOne^2 h^{-2}\normL{\ei_{x_i}}{K}^2
			= \invCoefOne h^{-2}\sum_{i=1}^{\nsd} \sum_{K\in\mesh}\left[\int_{K}|\ei_{x_i}|^2 dK \right]\\
			&= \invCoefOne^2 h^{-2}\sum_{i=1}^{\nsd} \left[\intOmega|\ei_{x_i}|^2 d\Omega \right]
			= \invCoefOne^2 h^{-2}\intOmega \left[\sum_{i=1}^{\nsd}|\ei_{x_i}|^2 \right]d\Omega
			= \invCoefOne^2 h^{-2}\normL{\grad \ei}{\Omega}.
		\end{align*}
		Finally, applying the Cauchy Schwarz inequality on $\glspar\kappa(\grad\ei_t,\grad\eh)$, we get,
		\begin{align*}
			|\glspar\kappa(\grad\ei_t,\grad\eh)| 
			&\leq \glspar\kappa\normL{\grad\ei_t}{\Omega}\normL{\grad\eh}{\Omega}
			\leq \glspar\kappa\invCoefOne h^{-1}\normL{\grad \ei}{\Omega}\normL{\grad\eh}{\Omega}\\
			&\leq \glspar\kappa\invCoefOne h^{-1}C_{a1}h^{k}\seminormH[k+1]{v}{\Omega}\normL{\grad\eh}{\Omega}\\
			&\leq C^8 \left(\glspar\kappa\normL{\grad\eh}{\Omega}\right)h^{k}\seminormH[k+1]{v}{\Omega}
			% &\leq \glspar\kappa \sum_{K\in\mathcal{K_h}}
			% &\leq \glspar\kappa\invCoefOne^2\normL{\grad\ei}{\Omega}\normL{\grad\eh}{\Omega}
		\end{align*}
		%9
		\item The next term $\glspar\kappa(\grad\ei,\grad\eh_t)$ similar to the previous one and can be estimated in the same way
		\begin{align*}
			|\glspar\kappa(\grad\ei,\grad\eh_t)| 
			&\leq \glspar\kappa\normL{\grad\eh}{\Omega}\normL{\grad\eh_t}{\Omega}
			\leq \glspar\kappa\invCoefOne h^{-1}\normL{\grad\ei}{\Omega}\normL{\grad\eh}{\Omega}\\
			&\leq \glspar\kappa\invCoefOne h^{-1}C_{a1}h^{k}\seminormH[k+1]{v}{\Omega}\normL{\grad\eh}{\Omega}\\
			&\leq C^9 \left(\glspar\kappa\normL{\grad\eh}{\Omega}\right)h^{k}\seminormH[k+1]{v}{\Omega}
		\end{align*}
	\end{itemize}
	Collating all the terms, we have,
	\begin{align*}
		\normV{\eh}^2 &\leq |\bformh(\ei,\eh)| \\
		&\leq C\Big(
		\glspar\normL{\eh_t}{\Omega} + \frac{1}{2}\normL\eh\bft
		+\glspar\normL{\grad\eh}{\Omega}
		+\kappa\normL{\grad\eh}{\Omega}\\
		&+\glspar\normL{\eh_t}{\Omega}
		+\glspar\normL{\grad\eh}{\Omega}
		+\glspar\normL{\grad \eh}{\Omega}
		+\glspar\normL{\eh_t}{\Omega}\\
		&+\glspar\kappa\normL{\grad\eh}{\Omega}
		+\glspar\kappa\normL{\grad\eh}{\Omega}
		\Big)h^{k}\seminormH[k+1]{v}{\Omega}\\
		&\leq C_2 \normV{\eh}h^{k}\seminormH[k+1]{v}{\Omega}.
	\end{align*}
	So we have
	\begin{align}
		\normV{\eh} \leq C_2 h^{k}\seminormH[k+1]{v}{\Omega}.
	\end{align}
	Going back to equation ~\eqref{eq:errors-triangle-ineq}, we get
	\begin{align}
		\normV{\er} 
		&\leq \normV{\eh} + \normV{\ei}\\
		&\leq (C_1 + C_2)h^{k}\seminormH[k+1]{v}{\Omega}\\
		&\leq C h^{k}\seminormH[k+1]{v}{\Omega}.
	\end{align}
	
	% Using the triangle inequality we get,
	% \begin{align*}
		%     \normV{e^h} = \normV{v-\vh} \leq \normV{v-\interp{v}} + \normV{\interp{v}-\vh}
		% \end{align*}
	% \begin{itemize}
		%     \item The first norm on the right hand side can be directly estimated using \ref{lemma:interp-estimate-in-Vh}.
		%     \begin{align*}
			%         \normV{v-\interp{v}} \leq Ch^{k}\seminormH[k+1]{v}{\Omega}
			%     \end{align*}
		%     \item The second norm can be estimated by making use of the coercivity property \ref{lemma:coercivity-stability} and the Galerkin orthogonality \ref{remark:galerkin-orthogonality}.
		%     \begin{align*}
			%     \mu_c \normV{\interp{v}-\vh}^2 
			%     &\leq \bformh(\interp{v}-\vh,\interp{v}-\vh)\\
			%     &\leq \bformh(\interp{v}-v,\interp{v}-\vh)+\bformh(v-\vh,\interp{v}-\vh)
			% \end{align*}
		% Since $\interp{v}-\vh \in \spaceVh$, therefore we have $\bformh(v-\vh,\interp{v}-\vh) = 0$ using the Galerkin orthogonality relation.
		% Thus,
		% \begin{align*}
			%     \mu_c \normV{\interp{v}-\vh}^2 
			%     &\leq \bformh(\interp{v}-v,\interp{v}-\vh)\\
			%     &\leq \mu_b \normVstar{\interp{v}-v}\normV{\interp{v}-\vh}
			% \end{align*}
		% which implies
		% \begin{align*}
			%     \normV{\interp{v}-\vh} 
			%     &\leq \frac{\mu_b}{\mu_c}\normVstar{\interp{v}-v}\\
			%     &\leq C_*\frac{\mu_b}{\mu_c}h^{k}\seminormH[k+1]{v}{\Omega}
			% \end{align*}
		% \end{itemize}
	% Therefore finally putting them together, we have 
	% \begin{align*}
		%     \normV{e^h} \leq \left(C + C_*\frac{\mu_b}{\mu_c} \right)h^{k}\seminormH[k+1]{v}{\Omega}
		% \end{align*}
	% which then proves the estimate.
\end{proof}

\subsection{Theorem \ref{theorem:a-posteriori-estimate} (A posteriori error estimate)} \label{sec:proof-a-posteriori}
\begin{proof}[Proof of Theorem \ref{theorem:a-posteriori-estimate}]
	The exact solution $v$ satisfies equation ~\eqref{eq:gls-abstract-for-exact-solution}. Equation ~\eqref{eq:gls-abstract-for-exact-solution} can also be written for test functions that belong to $V$ such that
	\begin{align}
		(\mathscr{L}v - F, w + \glspar\mathscr{L}w) &= 0 \ \ \forall w \in V\\
		\implies (\mathscr{L}v, w + \glspar\mathscr{L}w) &=  (F,w + \glspar\mathscr{L}w).
		\label{eq:gls-abstract-for-exact-solution-2}
	\end{align}
	From equation ~\eqref{eq:gls-abstract} and \eqref{def:discrete-variational-form}, we have
	\begin{align}
		(\mathscr{L}\vh, w + \glspar\mathscr{L}w) = \bformh(\vh,w).
		\label{def:discrete-variational-form-2}
	\end{align}
	Subtracting equation ~\eqref{def:discrete-variational-form-2} from \eqref{eq:gls-abstract-for-exact-solution-2}, we have
	%Now, the approximate solution $\vh$ does not satisfy this equation. Let us subtract $(\mathscr{L}\vh, w + \glspar\mathscr{L}w)$ from both side,
	\begin{align}
		\bformh(v-\vh,w) &=  (F,w + \glspar\mathscr{L}w) - \bformh(\vh,w).
	\end{align}
	The quantity on the left hand side is the weighted residual. Assuming $R\in V^*$, where $V^*$ is the dual space of $V$, this weighted residual can be written as a duality pairing $\langle \cdot,\cdot\rangle$ between $V$ and $V^*$.
	\begin{align*}\label{def:residual-calculation}
		\langle R,w\rangle &= \bformh(v-\vh,\wh) \\
		&=  (F,w + \glspar\mathscr{L}w) - \bformh(\vh,w)\\
		&= (F,w + \glspar\mathscr{L}w) \\
		&\qquad - \Big[ (\vht,\wh) + (\adv\cdot\grad\vh, \wh) + (\kappa\grad\vh,\grad\wh)\\
		&\qquad +\glspar(\vht,\wh_t) + \glspar(\vht,\adv\cdot\grad\wh)+\glspar(\grad\vht,\kappa\grad\wh)\\
		&\qquad +\glspar(\adv\cdot\grad\vh,\wh_t)+\glspar(\adv\cdot\grad\vh,\adv\cdot\grad\wh)-\glspar((\adv\cdot\grad\vh),\grad\cdot(\kappa\grad\wh))\\
		&\qquad +\glspar(\kappa\grad\vh,\grad\wh_t)-\glspar(\grad\cdot(\kappa\grad\vh), (\adv\cdot\grad\wh))+\glspar(\grad\cdot(\kappa\grad\vh),\grad\cdot(\kappa\grad\wh))\Big]\\
		&= (F,w + \glspar\mathscr{L}w) \\
		&\qquad -  (\vht,\wh) - (\adv\cdot\grad\vh, \wh) - \sum_{K\in\mesh}\left\{-(\grad\cdot\kappa\grad\vh),w)_K + \sum_{E\in \partial K}(\hat{n}\cdot\kappa\grad\vh, w)_E\right\}\\
		&\qquad -\glspar(\vht,\wh_t) - \glspar(\vht,\adv\cdot\grad\wh)-\glspar\sum_{K\in\mesh}\left\{-(\vht,\grad\cdot\kappa\grad w)_K + \sum_{E\in \partial K}(\vht, \hat{n}\cdot\kappa\grad w)_E\right\}\\
		&\qquad -\glspar(\adv\cdot\grad\vh,\wh_t)-\glspar(\adv\cdot\grad\vh,\adv\cdot\grad\wh)+\glspar((\adv\cdot\grad\vh),\grad\cdot(\kappa\grad\wh))\\
		&\qquad -\glspar\sum_{K\in\mesh}\left\{-(\grad\cdot\kappa\grad\vh, w_t)_K + \sum_{E\in \partial K}(\hat{n}\cdot\kappa\grad\vh, w_t)_E\right\}\\
		&\qquad+\glspar(\grad\cdot(\kappa\grad\vh), (\adv\cdot\grad\wh))-\glspar(\grad\cdot(\kappa\grad\vh),\grad\cdot(\kappa\grad\wh))\\
		&= (F,w + \glspar\mathscr{L}w)- \sum_{K\in\mesh}\left((\vht+\adv\cdot\grad\vh - \grad\cdot\grad\vh),w\right)_K\\
		&\qquad - \glspar\sum_{K\in\mesh}\left((\vht+\adv\cdot\grad\vh - \grad\cdot\grad\vh),w_t\right)_K - \glspar\sum_{K\in\mesh}\left((\vht+\adv\cdot\grad\vh - \grad\cdot\grad\vh),\adv\cdot\grad w\right)_K\\
		&\qquad + \glspar\sum_{K\in\mesh}\left((\vht+\adv\cdot\grad\vh - \grad\cdot\grad\vh),\grad\cdot\kappa\grad w\right)_K\\
		&\qquad -\sum_{E\in\edgeset} \mathbb{J}(\hat{n}\cdot\kappa\nabla\vh, w)_E + \glspar \mathbb{J}(\vht,\hat{n}\cdot\kappa\grad w)_E + \glspar \mathbb{J}(\hat{n}\cdot\kappa\grad\vh,w_t)_E\\
		&= (F,w + \glspar\mathscr{L}w) - \sum_{K\in\mesh}\left(\mathscr{L}\vh, w + \glspar\mathscr{L}w\right)_K \\&\qquad-\sum_{E\in\edgeset} \mathbb{J}(\hat{n}\cdot\kappa\nabla\vh, w + \glspar w_t)_E+ \glspar \mathbb{J}(\vht,\hat{n}\cdot\kappa\grad w)_E
	\end{align*}
	Now, the term $\glspar \mathbb{J}(\vht,\hat{n}\cdot\kappa\grad w)_E$ is zero, since $\hat{n}\cdot\kappa\grad w$ is in fact continuous across elements. Therefore the residual is
	\begin{align}
		\langle R,w\rangle &= \sum_{K\in\mesh}\left(F - \mathscr{L}\vh, w + \glspar\mathscr{L}w\right)_K-\sum_{E\in\edgeset} \mathbb{J}((\hat{n}\cdot\kappa\nabla\vh), w+w_t)_E\\
		&= \sum_{K\in\mesh}\left(r_K, w + \glspar\mathscr{L}w\right)_K-\sum_{E\in\edgeset} (j_E, w+w_t)_E.
	\end{align}
	Where the \textit{domain} and \textit{edge} residuals $r_K:\Omega \rightarrow \mathbb{R}$ and $j_E:\Omega\rightarrow \mathbb{R}$ are given by
	\begin{align}
		r|_K &= f - u^h_t - \mathbf{a}\cdot\nabla u^h + \kappa \nabla^2 u^h \qquad \text{on every } K \in \mesh,\\
		j|_E &= \begin{cases}
			-\mathbb{J}_E ( \hat{\mathbf{n}}_E\cdot\kappa \nabla u^h, v ) & \text{if }E \in \mathcal{E}_{\Omega}\\
			0 & \text{if } E \in \mathcal{E}_{\Gamma_D}.
		\end{cases}
	\end{align}
	% or,
	% \begin{align}
		%     \langle R,w\rangle &= \sum_{K\in\mesh}\left(r_K, w + \glspar\mathscr{L}w\right)_K-\sum_{E\in\edgeset} (j_E, w+w_t)_E
		% \end{align}
	By Galerkin orthogonality, we have
	\begin{align}
		\langle R,\interpolant w\rangle &= 0 \ \ \wh \in \spaceVh .
	\end{align}
	Suppose, $\phi = w + \glspar\mathscr{L}w$ and $\psi = w + w_t$. Then,
	\begin{align*}
		\langle R, w\rangle &= \langle R,w - \interpolant w\rangle\\
		&=\sum_{K\in\mesh}\left(r_K, \phi - \interpolant\phi\right)_K-\sum_{E\in\edgeset} (j_E, \psi-\interpolant \psi)_E\\
		&\leq \sum_{K\in\mesh} \normL{r_K}{K} C_1 h_K \normL{\grad \phi}{K} +\sum_{E\in\edgeset} \normL{j_E}{E}C_2 h_E^{1/2}\normL{\grad \psi}{E}\\
		&\leq \max(C_1, C_2) \left[\sum_{K\in\mesh}h_K^2\normL{r_K}{K}^2 + \sum_{E\in\edgeset} h_E\normL{j_E}{E}^2\right]^{\frac{1}{2}}
		\left[\sum_{K\in\mesh} \normL{\grad \phi}{K}^2 +\sum_{E\in\edgeset} \normL{\grad \psi}{E}^2\right]^{\frac{1}{2}}
	\end{align*}
	Now, because of shape regularity of $\mesh$,
	\begin{align*}
		\sum_{K\in\mesh} \normL{\grad \phi}{K}^2 
		&\leq 
		\sum_{K\in\mesh} \left( \normL{\grad w}{K} + \glspar\normL{\grad w_t}{K} + \glspar\normL{\grad (\adv\cdot\grad w)}{K} + \glspar\normL{\grad (\grad\cdot\kappa\grad w)}{K} \right)\\
		&\leq
		\sum_{K\in\mesh} \left( 1 + \glspar C_1 h^{-1} + \glspar C_2 \normL[\infty]{\adv}{K} h^{-1}+ \glspar C_3 \kappa h^{-2}\right)\normL{\grad w}{K}\\
		&\leq
		\sum_{K\in\mesh} C\normL{\grad w}{K}\\
		&\leq
		\sum_{K\in\mesh} C_{h_1}\normL{\grad w}{\Omega}.
	\end{align*}
	Similarly,
	\begin{align*}
		\sum_{E\in\edgeset} \normL{\grad \psi}{E}^2
		&\leq
		\sum_{K\in\mesh} C_{h_2}\normL{\grad w}{\Omega}.
	\end{align*}
	Combining,
	\begin{align*}
		\langle R,w\rangle \leq \max (C_1,C_2)(C_{h_1}+C_{h_2})\left[\sum_{K\in\mesh}h_K^2\normL{r_K}{K}^2 + \sum_{E\in\edgeset} h_E\normL{j_E}{E}^2\right]^{\frac{1}{2}}\normL{\grad w}{\Omega}
	\end{align*}
	or,
	\begin{align*}
		\sup \frac{1}{\normL{\grad w}{\Omega}} \langle R,w\rangle 
		&\leq
		\max (C_1,C_2)(C_{h_1}+C_{h_2})\left[\sum_{K\in\mesh}h_K^2\normL{r_K}{K}^2 + \sum_{E\in\edgeset} h_E\normL{j_E}{E}^2\right]^{\frac{1}{2}}\\
		&\leq
		C\left(\sum_{K\in\mesh}\eta_K^2\right)^{\frac{1}{2}}.
	\end{align*}
\end{proof}


\subsection{Corollary \ref{lemma:interp-boundary-estimate}} \label{sec:proof-interp-boundary}
\begin{proof}[Proof of Corollary \ref{lemma:interp-boundary-estimate}]
	Using \eqref{estimate:sobolev-interp}, the boundary norm $\normL{v-\interp{v}}{\bft}$ can also be estimated in terms of $\seminormH[k+1]{v}{\stDom}$ as follows.
	\begin{align*}
	\normL{v-\interp{v}}{\bft}^2 &
	\leq \normL{v-\interp{v}}{\partial \stDom}^2
	= \Xsum_{\substack{K\in\mesh \\ \partial K \cap \partial \stDom}}\normL{v-\interp{v}}{\partial K \cap \partial \stDom}^2\\
	&\leq \Xsum_{\substack{K\in\mesh}}\normL{v-\interp{v}}{\partial K}^2
	\end{align*}
	At this point, we make use of the trace inequality \cite{di2011mathematical, verfurth2013posteriori} defined for each element $K$ in the mesh,
	\begin{align}
	\normL{v-\interp{v}}{\partial K} \leq \traceConstant \left( h_K^{-1}\normL{v-\interp{v}}{K}^2 + h_K\normL{\grad(v-\interp{v})}{K}^2 \right)^{\frac{1}{2}}
	\label{estimate:scaled-trace-ineq-for-interp-error}
	\end{align}
	Now both $\normL{v-\interp{v}}{K}^2$ and $\normL{\grad(v-\interp{v})}{K}^2$ on the right hand side of \eqref{estimate:scaled-trace-ineq-for-interp-error} can be estimated with respect to $\seminormH[k+1]{v}{\stDom}$.
	\begin{align*}
	\normL{v-\interp{v}}{\bft}^2 
	&\leq \Xsum_{\substack{K\in\mesh}}\normL{v-\interp{v}}{\partial K}^2\\
	&\leq \traceConstant^2 \left[\Xsum_{\substack{k\in\mesh}}\left( h_K^{-1}\normL{v-\interp{v}}{K}^2 + h_K\normL{\grad(v-\interp{v})}{K}^2 \right)  \right]
	\end{align*}
	Assuming $h = \max \{h_K | K \in \mesh\}$, the shape regularity of the mesh $\mesh$ implies that there exists a constant $\shapeRegularConst$ such that for each element $K$ in $\mesh$
	\begin{align*}
	\Xsum_{\substack{K\in\mesh}}h_K^{-1}\normL{v-\interp{v}}{K}^2 
	&\leq \shapeRegularConst h^{-1}\normL{v-\interp{v}}{\stDom}^2
	\leq \shapeRegularConst h^{-1}\approxConstant^2 h^{2(k+1-0)}|v|_{H^{k+1}(\stDom)}^2\\
	&=\shapeRegularConst \approxConstant^2 h^{2k+1}|v|_{H^{k+1}(\stDom)}^2
	\end{align*}
	And similarly
	\begin{align*}
	\Xsum_{\substack{K\in\mesh}}h_K\normL{\grad(v-\interp{v})}{K}^2
	&\leq h\normL{\grad(v-\interp{v})}{\stDom}^2
	\leq h\approxConstant^2 h^{2(k+1-1)}|v|_{H^{k+1}(\stDom)}^2\\
	&\leq \approxConstant^2 h^{2k+1}|v|_{H^{k+1}(\stDom)}^2
	\end{align*}
	Combining, we get
	\begin{align}
	\normL{v-\interp{v}}{\bft}^2 
	&\leq \traceConstant^2 \approxConstant^2  \left( \shapeRegularConst + 1\right)h^{2k+1}|v|_{H^{k+1}(\stDom)}^2\\
	\implies\normL{v-\interp{v}}{\bft} 
	&\leq C_{a\Gamma}h^{k+\frac{1}{2}}|v|_{H^{k+1}(\stDom)}.
	\end{align}
\end{proof}

==> sections/6_proofs_new.tex <==
\section{Proofs for \secref{sec:math-formulation}}

\subsection{\lemref{lemma:boundedness} (Boundedness)}\label{sec:proof-boundedness}
\begin{proof}[Proof of \lemref{lemma:boundedness}]
	A reminder from \eqref{def:discrete-bilinear-form} that 
	\begin{align*}
	\bformh(\uh,\vh) &= (\uht,\vh) + (\adiv\uh, \vh) + (\visco\grad\uh,\grad\vh) +\innerh{\glspar \opLT \uh}{\opLT \vh}.
	\end{align*}
	Using $ \divergence \adv = 0 $, and assuming  $ \norm{\adv}_{\infty} = \theta $, we can rewrite the second term as
	\begin{align*}
	(\adiv\uh, \vh) = (\adiv\uh, \vh) + \inner{(\divergence \adv)\uh}{\vh} = \inner{\divergence (\uh \adv^T)}{\vh} &= -\inner{\uh \adv^T}{\grad \vh} \\
	&\leq \norm{\uh}\norm{\adv}_{\infty}\norm{\grad \vh} \\
	&= \theta \norm{\uh}\norm{\grad\vh},
	\end{align*}
	where we have used the H\"{o}lder's inequality with $ p=2,\ q=\infty,\ r=2 $. So, we have
	\begin{align*}
	|\bformh(\uh,\vh)| &\leq \norm{\uht}\norm{\vh} + \theta \norm{\uh} \norm{\grad \vh} + \visco\norm{\grad \uh} \norm{\grad\vh} + \normh{\glspar^{\halfnice} \opLT\uh} \normh{\glspar^{\halfnice} \opLT\vh} \\
	&\leq \left[ \norm{\uht}^2 + \theta^2 \norm{\uh}^2 + \visco^2 \norm{\grad \uh}^2+ \normh{\glspar^{\halfnice} \opLT\uh}^2 \right]^{\halfnice}  \\
	&\qquad\qquad\qquad\qquad\qquad\qquad \times \left[ \norm{\vh}^2 + 2\normh{\grad \vh}^2 + \normh{\glspar^{\halfnice} \opLT \vh}^2 \right]^{\halfnice}.
	\end{align*}
	Now, we have the trace inequalities \cite{evans2022partial, brenner2007mathematical, verfurth2013posteriori},
	\begin{align}
	\norm{\uh}_{\bft} \leq C \normH[1]{\uh}{\stDom} \leq  \traceConstant \norm{\uh},
	\end{align}
	where we have used the Poincar\'{e}'s inequality in the last step. Now, suppose $ \traceConstantMin $ is a constant such that $ \norm{\uh}_{\bft} = \traceConstantMin \norm{\uh} $ holds. Then, using $ \lambda = (\traceConstantMin)^{-1}$, we have
	\begin{align*}
	|\bformh(\uh,\vh)| &\leq \left[ \norm{\uht}^2 + \theta^2 {\lambda}^2 \norm{\uh}_{\bft}^2 + \visco^2 \norm{\grad \uh}^2+ \normh{\glspar^{\halfnice} \opLT\uh} \right]^{\halfnice}  \\
	&\qquad\qquad\qquad\qquad\qquad\qquad \times \left[ {\lambda}^2 \norm{\vh}_{\bft}^2 + 2\normh{\grad \vh}^2 + \normh{\glspar^{\halfnice} \opLT \vh} \right]^{\halfnice} \\
	&\leq \mu_b \normVhstar{\uh}\normVh{\vh},
	\end{align*}
	where $  $
	\begin{align*}
	\mu_b &= c_1 \times c_2, \\
	c_1 &=  \max \left\{ 1, (\theta {\lambda})^2, \visco^2 \right\}, \\
	c_2 &= \max \left\{ 2, ({\lambda})^2 \right\}.
	\end{align*}
\end{proof}


\subsection{\lemref{lemma:coercivity-stability} (Coercivity)}\label{sec:proof-coercivity}
\begin{proof}[Proof of \lemref{lemma:coercivity-stability}]
	From \eqref{def:discrete-bilinear-form}, we have
	\begin{align*}
	\bformh(\uh,\uh) &= \inner{\uht}{\uh} + \inner{\adiv \uh}{\uh} + \inner{\visco \grad \uh}{\grad \uh} +\innerh{\glspar \opLT \uh}{\opLT \uh}. \end{align*}
	The first term can be written as
	\begin{align*}
	\inner{\uht}{\uh} &= \intSpaceTime \uh \uht \  dt\ d\spDom = \half \intSpaceTime \frac{\partial}{\partial t} (\uh^2) dt d\spDom = \half \intSpace \left[ \uh^2(\xvec, T) - \uh^2(\xvec,0) \right]\ d\spDom \\
	&= \half \intSpace \uh^2(\xvec, T) \ d\spDom \\
	&= \halfnice \norm{\uh}_{\bft}^2.
	\end{align*}
	As shown in the proof of \lemref{lemma:boundedness} (\ref{sec:proof-boundedness}), using $ \divergence \adv = 0 $, the second term can be written as
	\begin{align*}
	\inner{\adiv \uh}{\uh} 
	&= -\inner{\uh \adv^T}{\grad \uh} \\
	&= -\inner{\uh}{\adiv \uh}.
	\end{align*}
	Which implies $ 2\inner{\adiv \uh}{\uh}  = 0 $. So, we have
	\begin{align*}
	\bformh(\uh,\uh) &= \halfnice \norm{\uh}_{\bft}^2 + \visco \norm{\grad \uh}^2 +\normh{\glspar^{\halfnice} \opLT \uh}^2 \\
	&\geq \mu_c\ \normVh{\uh}^2,
	\end{align*}
	where $ \mu_c = \min \left\{ \halfnice,\ \visco \right\} $.
\end{proof}


\subsection{\cororef{lemma:interp-boundary-estimate}} \label{sec:proof-interp-boundary}
\begin{proof}[Proof of \cororef{lemma:interp-boundary-estimate}]
	We make use of the trace inequality \cite{di2011mathematical, verfurth2013posteriori} defined for each element $K$ in the mesh,
	\begin{align*}
	\normL{v-\interp{v}}{\partial K}^2 &\leq C_E \left( h_K^{-1}\normL{v-\interp{v}}{K}^2 + h_K\normL{\grad(v-\interp{v})}{K}^2 \right) \\
	&\leq  C_E \left( h_K^{-1}{\approxConstant}_0^2 \he^{2(k+1-0)}|v|_{H^{k+1}(K)}^2 + h_K {\approxConstant}_1^2 \he^{2(k+1-1)}|v|_{H^{k+1}(K)}^2 \right) \\	
	&\leq C_E ({\approxConstant}_0^2 + {\approxConstant}_1^2) \he^{2k+1} |v|_{H^{k+1}(K)}^2 \\
	&= C_{aE}^2 \he^{2k+1} |v|_{H^{k+1}(K)}^2,
	\end{align*}
	where $ C_{aE} = \sqrt{C_E ({\approxConstant}_0^2 + {\approxConstant}_1^2)} $.
\end{proof}

\subsection{\lemref{lemma:interp-estimate-in-Vh}} \label{proof:interp-estimate-vh}
\begin{proof}[Proof of \lemref{lemma:interp-estimate-in-Vh}]
	Suppose, $ \ei = \interp{u} - u $, and assume $ \glsparMax = \max_K \glspar_K $. Then we have
	\begin{align*}
	\normVh{\ei}^2 &= \left[\normVExpanded{\ei}\right] \\
	&\leq {\approxConstant}_{\Gamma}^2 h^{2k+1}\seminormH[k+1]{u}{\stDom}^2  + {\approxConstant}_1^2 h^{2k} \seminormH[k+1]{u}{\stDom}^2 + \glsparMax \elmsum \normElm{\residual{\ei}}^2 \\
	&\leq \left({\approxConstant}_{\Gamma}^2 h^{2k+1}  + {\approxConstant}_1^2 h^{2k}\right)\seminormH[k+1]{u}{\stDom}^2 + \glsparMax \elmsum \left[ \normElm{\partial_t \ei} + \normElm{\adiv \ei} + \visco\normElm{\laplacian \ei} \right]^2 \\
	&\leq \left({\approxConstant}_{\Gamma}^2 h^{2k+1}  + {\approxConstant}_1^2 h^{2k}\right)\seminormH[k+1]{u}{\stDom}^2 + \glsparMax \elmsum \left[ {\approxConstant}_1(1+\norm{\adv}_{\infty}) \he^{k} \seminormH[k+1]{u}{K} + \visco{\approxConstant}_{2} \he^{k-1} \seminormH[k+1]{u}{K} \right]^2 \\
	&\leq \left({\approxConstant}_{\Gamma}^2 h^{2k+1}  + {\approxConstant}_1^2 h^{2k}\right)\seminormH[k+1]{u}{\stDom}^2 + C\glsparMax \elmsum \left( \he + c \right)^2 \he^{2(k-1)} \seminormH[k+1]{u}{K}^2 \\
	&\leq \left({\approxConstant}_{\Gamma}^2 h^{2k+1}  + {\approxConstant}_1^2 h^{2k}\right)\seminormH[k+1]{u}{\stDom}^2 + C\glsparMax \left( h + c \right)^2 h^{2(k-1)} \elmsum  \seminormH[k+1]{u}{K}^2 \\
	&\leq \left({\approxConstant}_{\Gamma}^2 h^{2k+1}  + {\approxConstant}_1^2 h^{2k} + C\glsparMax \left( h + c \right)^2 h^{2(k-1)}\right)\seminormH[k+1]{u}{\stDom}^2 \\
	&\leq \left[C_1 h^3 + C_2 h^2 + C_3 \glsparMax (h+c)^2 \right] h^{2(k-1)} \seminormH[k+1]{u}{\stDom}^2.
	\end{align*}
	Assuming $ \glsparMax = \gamma h^2,\ \gamma>0 $, (i.e., assuming a diffusive limit, see Remark \ref{remark:stabilization}), we have
	\begin{align*}
	\normVh{\ei}^2 &\leq \left[C_1 h + C_2 + C_3 \gamma (h+c)^2 \right] h^{2k} \seminormH[k+1]{u}{\stDom}^2 \\
	&\leq (C(h))^2 h^{2k} \seminormH[k+1]{u}{\stDom}^2.
	\end{align*}
	Thus, we have the required estimate.
\end{proof}

\subsection{\thmref{theorem:a-priori-estimate} (A priori error estimate)} \label{sec:proof-a-priori}
\begin{proof}[Proof of \thmref{theorem:a-priori-estimate}]
	Define $\er = \uh - u$, $\eh = \uh-\interpolant u$ and $\ei = \interpolant u - u$. These three quantities are related as
	\begin{align}
	\er &=  \uh - u \\ &= \uh - \interp{u} + \interp{u} - u \\ &= \eh + \ei
	\end{align}
	By triangle inequality
	\begin{align}
	\normVh{\er} \leq \normVh{\eh} + \normVh{\ei}
	\label{eq:errors-triangle-ineq}
	\end{align}
	From \lemref{lemma:interp-estimate-in-Vh}, the estimate on $\normVh{\ei}$ is already known, i.e.,
	\begin{align}
	\normVh{\ei}\leq C_1 h^k|v|_{H^{k+1}(\stDom)}
	\end{align}
	Now we try to estimate $\normVh{\eh}$ using $ \bformh(\eh, \eh) $. We have
    \begin{align*}
			\mu_c \normVh{\eh}^2 
			&\leq \bformh(\eh,\eh) = \bformh(\er-\ei,\eh) = \bformh(\er,\eh)-\bform(\ei,\eh) = -\bform(\ei,\eh) \leq |\bform(\ei,\eh)| \leq \mu_b \normVhstar{\ei} \normVh{\eh},
	\end{align*}
    i.e,
    \begin{align*}
        \normVh{\eh} \leq (\nicefrac{\mu_b}{\mu_c}) \normVhstar{\ei} \leq C_2 h^{k}\seminormH[k+1]{v}{\stDom}.
    \end{align*}
	Substituting in ~\eqref{eq:errors-triangle-ineq}, we get
	\begin{align}
	\normVh{\er} 
	&\leq \normVh{\eh} + \normVh{\ei}\\
	&\leq (C_1 + C_2)h^{k}\seminormH[k+1]{v}{\stDom}\\
	&\leq C h^{k}\seminormH[k+1]{v}{\stDom}.
	\end{align}
\end{proof}

\subsection{\thmref{theorem:a-posteriori-estimate} (A posteriori error estimate)} \label{sec:proof-a-posteriori}
\begin{proof}[Proof of \thmref{theorem:a-posteriori-estimate}]
	The proof below closely follows the arguments presented in Section 1.4 of \cite{verfurth2013posteriori}.
	We can rewrite ~\eqref{eq:gls-abstract-for-exact-solution} and \eqref{eq:exact-solution-discrete-form} for any $ v \in \spaceV $ as
	\begin{subequations}
		\begin{align}
		\innerh{\opLT u - F}{v + \glspar\opLT v} &= 0 \ \ \forall v \in \spaceV, \\
		\implies \bformh(u, v) &= \lformh(v) \ \ \forall v \in \spaceV.
		\end{align}
	\end{subequations}
	Let us denote the strong residual as $ R(u) = \opLT u - F $, and the weak residual as
	\begin{align}
	\innerh{R(\uh)}{v} &= \lformh(v) - \bformh(\uh,v) \\
	&= \bformh(u,v) - \bformh(\uh,v) \\
	&= \bformh(u-\uh,v).
	\end{align}
	So, we have
	\begin{align}
	\innerh{R(\uh)}{v} &= \lformh(v) - \bformh(\uh,v) \\
	&= \innerh{F}{v + \glspar \opLT v} - \left[ (\uht, v) + (\adiv\uh,  v) + (\visco\grad\uh,\grad v) +\innerh{\glspar \opLT \uh}{\opLT  v} \right] \\
	&= \elmsum \inner{F}{v + \glspar \opLT v}_K - \left[ (\uht, v)_K + (\adiv\uh,  v)_K + (\visco\grad\uh,\grad v)_K +\inner{\opLT \uh}{\glspar \opLT  v}_K \right] \\
	&= \elmsum \inner{F}{v + \glspar \opLT v}_K \\ &\qquad\qquad - \left[ (\uht, v)_K + (\adiv\uh,  v)_K - (\visco\laplacian\uh,v)_K + \Xsum_{E \in \partial K} \inner{\visco \ddiv{\normalvec}}{v} +\inner{\opLT \uh}{\glspar \opLT  v}_K \right] \\
	&= \elmsum \inner{F}{v + \glspar \opLT v}_K - \left[ \inner{\opLT \uh}{v}_K + \inner{\opLT \uh}{\glspar \opLT  v}_K + \Xsum_{E \in \partial K} \inner{\visco \ddiv{\normalvec}}{v} \right] \\
	&= \elmsum \inner{F - \opLT \uh}{v + \glspar \opLT v}_K - \edgesum \inner{\visco \jump(\ddiv{\normalvec}\uh)}{v}_E.
	\end{align}
	Define the elemental residual as $ r = (F - \opLT \uh) |_K $ and the jump on an edge as $ j = -(\visco \jump(\ddiv{\normalvec}\uh))|_E$. Then we have
	\begin{align} \label{eq:aposter-weak-res-v}
	\innerh{R(\uh)}{v} &= \elmsum \left[\inner{r}{v}_K + \inner{r}{\glspar \opLT v}_K\right] + \edgesum \inner{j}{v}_E \ \text{for any}\ v \in \spaceV
	\end{align}
	Now, by Galerkin orthogonality, we have
	\begin{align}
	\innerh{R(\uh)}{\vh} = 0 \ \text{for any}\ \vh \in \spaceVh.
	\end{align}
	So, using $ \vh \in \spaceVh \subset \spaceV $ in \eqref{eq:aposter-weak-res-v}, we have
	\begin{align} \label{eq:aposter-weak-res-vh}
	0 &= \elmsum \left[\inner{r}{\vh}_K + \inner{r}{\glspar \opLT \vh}_K\right] + \edgesum \inner{j}{\vh}_E \ \forall \vh \in \spaceVh.
	\end{align}
	Subtracting \eqref{eq:aposter-weak-res-vh} from \eqref{eq:aposter-weak-res-v}, we have for any $ v \in \spaceV $ and every $ \vh \in \spaceVh $,
	\begin{align} 
	\innerh{R(\uh)}{v} &= \elmsum \left[\inner{r}{v-\vh}_K + \inner{r}{\glspar \opLT (v-\vh)}_K\right] + \edgesum \inner{j}{(v-\vh)}_E \\
	&\leq \elmsum \normElm{r} \left(\normElm{v-\vh} + \glsparMax \normElm{\opLT (v-\vh)} \right) + \edgesum \norm{j}_E \norm{v-\vh}_E.
	\end{align}
	Now, choosing $ \vh = \interp{v} $ and using the estimates from \eqref{estimate:sobolev-interp}, we have
	\begin{align}
	\innerh{R(\uh)}{v} &\leq \elmsum \normElm{r} \left( C_{a0}\he^{k+1} + \glsparMax C_{a2} \he^{k-1} \right) \seminormH[k+1]{v}{K} + \edgesum \norm{j}_E C_{a \Gamma} \he^{k+\half}  \seminormH[k+1]{v}{E}.
	\end{align}
	Assuming $ \glsparMax = \gamma h^2,\ \gamma>0 $, (i.e., assuming a diffusive limit, see \remref{remark:stabilization}), we have
	\begin{align}
	\innerh{R(\uh)}{v} &\leq \elmsum \he^{k+1} \normElm{r} \left( C_{a0} + \gamma C_{a2} \right) \seminormH[k+1]{v}{K} + \edgesum \norm{j}_E C_{a \Gamma} h_E^{k+\half}  \seminormH[k+1]{v}{E}.
	\end{align}
	Using Cauchy-Schwarz inequality, we have
	\begin{align}
	\innerh{R(\uh)}{v} &\leq \ C \  \left[\elmsum \he^{2(k+1)} \normElm{r}^2 + 
	\edgesum h_E^{2k+1} \norm{j}_E^2 \right]^{\halfnice} \\
	&\qquad\qquad \times \left[\elmsum \seminormH[k+1]{v}{K}^2 + \edgesum \seminormH[k+1]{v}{E}^2 \right]^{\halfnice}.
	\end{align}
	The first term in the brackets on the right hand side can be bounded as
	\begin{align*}
	\left[\elmsum \he^{2(k+1)} \normElm{r}^2 + 
	\edgesum h_E^{2k+1} \norm{j}_E^2 \right]^{\halfnice} &\leq \left[\elmsum \left(\he^{2(k+1)} \normElm{r}^2 + 
	\Xsum_{E \in \mathcal{E}_K} h_E^{2k+1} \norm{j}_E^2\right) \right]^{\halfnice} \\
	&\leq \left[\elmsum h^{2k} \left(\he^{2} \normElm{r}^2 + 
	\Xsum_{E \in \mathcal{E}_K} h_E \norm{j}_E^2\right) \right]^{\halfnice} \\
	&\leq h^{k} \left(\elmsum {\etaElm}^2\right)^{\halfnice}, \\
	&= h^k \etaFull
	\end{align*}
	where $ h $ is defined as
	\begin{align}
	h = \max \left\{ \max_{K \in \mesh} h_K, \ \ \max_{E \in \edgeset} h_E  \right\}.
	\end{align}
	Also, due to shape regularity, we can write
	\begin{align}
	\left[\elmsum \seminormH[k+1]{v}{K}^2 + \edgesum \seminormH[k+1]{v}{E}^2 \right]^{\halfnice} \leq C \seminormH[k+1]{v}{\stDom}.
	\end{align}
	Thus, we have
	\begin{align}
	\innerh{R(\uh)}{v} 
	&\leq C \etaFull h^k \seminormH[k+1]{v}{\stDom}.
	\end{align}
	Now, using $ \innerh{R(\uh)}{v} = \bformh(u-\uh, v) $, we also have
	\begin{align}
	\innerh{R(\uh)}{v} &= \bformh(u-\uh, v) \\
	&=  \bformh(u-\uh, v) -  \bformh(u-\uh, \vh) \quad \text{(by Galerkin orthogonality)} \\
	&= \bformh(u-\uh, v-\vh) \\
	&\leq \mu_b \normVhstar{u-\uh}\normVh{v-\vh}.
	\end{align}
	Once again, choosing $ \vh = \interp{v} $, we have
	\begin{align}
	\innerh{R(\uh)}{v} &\leq \mu_b \normVhstar{u-\uh} C_{a0} h^k \seminormH[k+1]{v}{\stDom} \\
	\implies \oneOver{\mu_b C_{a0} h^k \seminormH[k+1]{v}{\stDom}} \innerh{R(\uh)}{v} &\leq \normVhstar{u-\uh}.
	\end{align}
	Using a similar argument as in \cite{verfurth2013posteriori} (Theorem 1.5), we can say
	\begin{align}
	\normVhstar{u-\uh} &= \sup_{v \in \spaceV \backslash \{0\}} \oneOver{\mu_b C_{a0} h^k \seminormH[k+1]{v}{\stDom}} \innerh{R(\uh)}{v} \\
	&\leq \oneOver{\mu_b C_{a0} h^k \seminormH[k+1]{v}{\stDom}} C \etaFull h^k \seminormH[k+1]{v}{\stDom} \\
	&\leq C\etaFull.
	\end{align}
\end{proof}

